Efficient reduction of Kappa models by static inspection of the rule-set

When designing genetic circuits, the typical primitives used in major existing modelling formalisms are gene interaction graphs, where edges between genes denote either an activation or inhibition relation. However, when designing experiments, it is important to be precise about the low-level mechanistic details as to how each such relation is implemented. The rule-based modelling language Kappa allows to unambiguously specify mechanistic details such as DNA binding sites, dimerisation of transcription factors, or co-operative interactions. However, such a detailed description comes with complexity and computationally costly execution. We propose a general method for automatically transforming a rule-based program, by eliminating intermediate species and adjusting the rate constants accordingly. Our method consists of searching for those interaction patterns known to be amenable to equilibrium approximations (e.g. Michaelis-Menten scheme). The reduced model is efficiently obtained by static inspection over the rule-set, and it represents a particular theoretical limit of the original model. The Bhattacharyya distance is proposed as a metric to estimate the reduction error for a given observable. The tool is tested on a detailed rule-based model of a $\lambda$-phage switch, which lists $96$ rules and $16$ agents. The reduced model has $11$ rules and $5$ agents, and provides a dramatic reduction in simulation time of several orders of magnitude.

==> MyRef <==
@article{ptashne1986genetic,
  title={A genetic switch: Gene control and phage. lambda},
  author={Ptashne, Mark},
  year={1986},
  publisher={Palo Alto, CA (US); Blackwell Scientific Publications}
}

@book{myers2011engineering,
  title={Engineering genetic circuits},
  author={Myers, Chris J},
  year={2011},
  publisher={CRC Press}
}

@article{ptashne2001genes,
  title={Genes \& signals},
  author={Ptashne, Mark A},
  year={2001},
  publisher={Cold Spring Harbor Laboratory Press}
}


@inproceedings{reconstruction,
  author    = {Tatjana Petrov and  Jerome Feret and Heinz Koeppl},
  title     = {Reconstructing species-based dynamics from reduced stochastic rule-based models},
  booktitle = {Winter Simulation Conference},
  year      = {2012},
  pages     = {},
  ee        = {},
  crossref  = {},
  bibsource = {}
}

@inproceedings{approx,
  author    = {Tatjana Petrov and Heinz Koeppl},
  title     = {Approximate reductions of rule-based models},
  booktitle = {European Control Conference},
  year      = {2013},
  pages     = {},
  ee        = {},
  crossref  = {},
  bibsource = {}
}

@article{Rizk,
  author    = {Fran\c{c}ois Fages and
               Aur{\'e}lien Rizk},
  title     = {On temporal logic constraint solving for analyzing numerical
               data time series},
  journal   = {Theor. Comput. Sci.},
  volume    = {408},
  number    = {1},
  year      = {2008},
  pages     = {55-65},
  ee        = {http://dx.doi.org/10.1016/j.tcs.2008.07.004},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}

@article{rewire,
author = {Caleb J. Bashor and Andrew A. Horwitz and Sergio G. Peisajovich and Wendell A. Lim},
title = {{Rewiring Cells: Synthetic Biology as a Tool to Interrogate the Organizational Principles of Living Systems}},
journal = {Annual Review of Biophysics},
volume = {39},
year = {2010},
pages = {515--537},
issue = {1},
doi = {10.1146/annurev.biophys.050708.133652},
masid = {38370071}
}



@INPROCEEDINGS{Alfaro01interfacetheories,
    author = {Luca De Alfaro and Thomas A. Henzinger},
    title = {Interface Theories for Component-based Design},
    booktitle = {},
    year = {2001},
    pages = {148--165},
    publisher = {Springer-Verlag}
}

@incollection{chapter,
   address     = {New York},
   affiliation = {EPFL},
   author      = {Hafner, Marc and Petrov, Tatjana and Lu, James and Koeppl, Heinz},
   booktitle   = {Design and {A}nalysis of {B}io-{M}olecular {C}ircuits},
   details     = {http://infoscience.epfl.ch/record/163582},
   editor      = {Koeppl, Heinz and Densmore, D. and di Bernardo, M. and Setti, Gianluca},
   keywords    = {model, robustness, LTL, parameter space},
   oai-id      = {oai:infoscience.epfl.ch:163582},
   oai-set     = {chapter},
   publisher   = {Springer},
   status      = {PUBLISHED},
   submitter   = {137075},
   title       = {Rational design of robust biomolecular circuits: from
                 specification to parameters},
   unit        = {LANOS},
   year        = 2011
}



@inproceedings{pnueli77,
  author    = {Amir Pnueli},
  title     = {The Temporal Logic of Programs},
  booktitle = {FOCS},
  year      = {1977},
  pages     = {46-57},
  ee        = {http://doi.ieeecomputersociety.org/10.1109/SFCS.1977.32},
  crossref  = {DBLP:conf/focs/FOCS18},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}


@article{nextgen,
    abstract = {{Synthetic biology is focused on the rational construction of biological systems based on engineering principles. During the field's first decade of development, significant progress has been made in designing biological parts and assembling them into genetic circuits to achieve basic functionalities. These circuits have been used to construct proof-of-principle systems with promising results in industrial and medical applications. However, advances in synthetic biology have been limited by a lack of interoperable parts, techniques for dynamically probing biological systems and frameworks for the reliable construction and operation of complex, higher-order networks. As these challenges are addressed, synthetic biologists will be able to construct useful next-generation synthetic gene networks with real-world applications in medicine, biotechnology, bioremediation and bioenergy.}},
    author = {Lu, Timothy K. and Khalil, Ahmad S. and Collins, James J.},
    booktitle = {Nat Biotech},
    citeulike-article-id = {6346105},
    citeulike-linkout-0 = {http://dx.doi.org/10.1038/nbt.1591},
    citeulike-linkout-1 = {http://dx.doi.org/10.1038/nbt.1591},
    citeulike-linkout-2 = {http://www.ncbi.nlm.nih.gov/pmc/articles/PMC2796205/},
    citeulike-linkout-3 = {http://view.ncbi.nlm.nih.gov/pubmed/20010597},
    citeulike-linkout-4 = {http://www.hubmed.org/display.cgi?uids=20010597},
    day = {09},
    doi = {10.1038/nbt.1591},
    issn = {1087-0156},
    journal = {Nature Biotechnology},
    keywords = {synthetic\_biology},
    month = dec,
    number = {12},
    pages = {1139--1150},
    pmcid = {PMC2796205},
    pmid = {20010597},
    posted-at = {2009-12-22 15:43:30},
    priority = {2},
    publisher = {Nature Publishing Group},
    title = {{Next-generation synthetic gene networks}},
    url = {http://dx.doi.org/10.1038/nbt.1591},
    volume = {27},
    year = {2009}
}



@article{sorger06,
    abstract = {{Physicochemical modelling of signal transduction links fundamental chemical and physical principles, prior knowledge about regulatory pathways, and experimental data of various types to create powerful tools for formalizing and extending traditional molecular and cellular biology.}},
    author = {Aldridge, Bree B. and Burke, John M. and Lauffenburger, Douglas A. and Sorger, Peter K.},
    citeulike-article-id = {921837},
    citeulike-linkout-0 = {http://dx.doi.org/10.1038/ncb1497},
    citeulike-linkout-1 = {http://dx.doi.org/10.1038/ncb1497},
    citeulike-linkout-2 = {http://view.ncbi.nlm.nih.gov/pubmed/17060902},
    citeulike-linkout-3 = {http://www.hubmed.org/display.cgi?uids=17060902},
    day = {01},
    doi = {10.1038/ncb1497},
    issn = {1465-7392},
    journal = {Nature Cell Biology},
    keywords = {nature\_sysbio\_08, systems\_biology},
    month = nov,
    number = {11},
    pages = {1195--1203},
    pmid = {17060902},
    posted-at = {2008-05-04 12:29:25},
    priority = {3},
    publisher = {Nature Publishing Group},
    title = {{Physicochemical modelling of cell signalling pathways}},
    url = {http://dx.doi.org/10.1038/ncb1497},
    volume = {8},
    year = {2006}
}



@article{hardtruth,
    author = {Kwok, Roberta},
    citeulike-article-id = {6607383},
    citeulike-linkout-0 = {http://dx.doi.org/10.1038/463288a},
    day = {21},
    doi = {10.1038/463288a},
    issn = {0028-0836},
    journal = {Nature},
    keywords = {commentary, overview, synthetic\_biology},
    month = jan,
    number = {7279},
    pages = {288--290},
    posted-at = {2010-02-24 09:52:59},
    priority = {5},
    title = {{Five hard truths for synthetic biology}},
    url = {http://dx.doi.org/10.1038/463288a},
    volume = {463},
    year = {2010}
}



@inproceedings{Fisher_synthesis,
  author    = {Ali Sinan K{\"o}ksal and
               Yewen Pu and
               Saurabh Srivastava and
               Rastislav Bod\'{\i}k and
               Jasmin Fisher and
               Nir Piterman},
  title     = {Synthesis of biological models from mutation experiments},
  booktitle = {POPL},
  year      = {2013},
  pages     = {469-482},
  ee        = {http://doi.acm.org/10.1145/2429069.2429125},
  crossref  = {DBLP:conf/popl/2013},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}

@MISC{Durrett,
    author = {Rick Durrett},
    title = {Probability: Theory and examples},
    year = {2011}
}

@book{norris97,
  added-at = {2011-05-09T23:10:52.000+0200},
  address = {Cambridge, UK},
  author = {Norris, J. R.},
  biburl = {http://www.bibsonomy.org/bibtex/25544e31bf4ad2b57f702536b978b64a4/josephausterwei},
  interhash = {a9011cd0840f0900986299ad5ece75f9},
  intrahash = {5544e31bf4ad2b57f702536b978b64a4},
  keywords = {imported},
  publisher = {Cambridge University Press},
  timestamp = {2011-05-09T23:10:52.000+0200},
  title = {Markov Chains},
  year = 1997
}

@book{Gray,
 author = {Gray, Robert M.},
 title = {Entropy and information theory},
 year = {1990},
 isbn = {0-387-97371-0},
 publisher = {Springer-Verlag New York, Inc.},
 address = {New York, NY, USA},
} 


@book{KS60:lump,
	Author = {Kemeny, John and Snell, James L.},
	Publisher = {Van Nostrand},
	Title = {Finite {M}arkov Chains},
	Year = {1960}}

@misc{norris,
      author = {Norris, James},
      title = {Probability and Measure},
      year = {2011},
      note = {\texttt{http://www.statslab.cam.ac.uk/~james/Lectures/pm2012.pdf}
}


@misc{anderson,
      author = {Anderson, David},
      title = {Introduction to Stochastic Processes with Applications in the Biosciences},
      year = {2011},
      note = {\texttt{http://www.math.wisc.edu/~anderson/605F11/Notes/StochBio.pdf}}
}


@article{journal,
	Author = {Jerome Feret and Heinz Koeppl and Tatjana Petrov},
	Date-Added = {2010-08-03 14:49:24 +0200},
	Date-Modified = {2010-08-03 14:49:24 +0200},
	Journal = {International Journal of Software and Informatics},
	Owner = {petrov},
	Title = {Stochastic fragments: A framework for the exact reduction of the stochastic semantics of rule-based models},
	Volume = {to appear},
	Year = {2013}}
	

@book{winskel,
 author = {Winskel, Glynn},
 title = {The formal semantics of programming languages: an introduction},
 year = {1993},
 isbn = {0-262-23169-7},
 publisher = {MIT Press},
 address = {Cambridge, MA, USA},
} 

@inproceedings{Scott71,
    abstract = {{Compilers for high-level languages are generally constructed to give the complete translation of the programs into machine language. As machines merely juggle bit patterns, the concepts of the original language may be lost or at least obscured during this passage. The purpose of a mathematical semantics is to give a correct and meaningful correspondence between programs and mathematical entities in a way that is entirely independent of an implementation. This plan is illustrated in a very elementary way in the introduction. Section II connects the general method with the usual idea of state transformations. The next section shows why the mathematics of functions has to be modified to accommodate recursive commands. Section IV explains the modification. Section V introduces the environments for handling variables and identifiers, and shows how the semantical equations define equivalence of programs. Section VI gives an exposition of the new type of mathematical function spaces that are required for the semantics of procedures when these are allowed in assignment statements. The conclusion traces some of the background of the project and points the way to future work.}},
    address = {Brooklyn, N.Y.},
    author = {Scott, Dana and Strachey, Christopher},
    booktitle = {Proceedings of the Symposium on Computers and Automata},
    citeulike-article-id = {5931338},
    citeulike-linkout-0 = {http://books.google.com/books?id=TekiAAAAMAAJ\&\#38;dq=70-185593\&\#38;q=\%22toward+a+mathematical+semantics+for+computer+languages\%22\#search\_anchor},
    editor = {Fox, Jerome},
    keywords = {1971, denotational, semantics},
    month = apr,
    pages = {19--46},
    posted-at = {2012-01-23 11:25:00},
    priority = {2},
    publisher = {Polytechnic Press},
    title = {{Toward A Mathematical Semantics for Computer Languages}},
    url = {http://books.google.com/books?id=TekiAAAAMAAJ\&\#38;dq=70-185593\&\#38;q=\%22toward+a+mathematical+semantics+for+computer+languages\%22\#search\_anchor},
    volume = {XXI},
    year = {1971}
}

%% This BibTeX bibliography file was created using BibDesk.
%% http://bibdesk.sourceforge.net/


%% Created for Petrov at 2011-11-14 10:21:42 +0100 


%% Saved with string encoding Unicode (UTF-8) 

@article{sachs05,
    abstract = {{Machine learning was applied for the automated derivation of causal influences in cellular signaling networks. This derivation relied on the simultaneous measurement of multiple phosphorylated protein and phospholipid components in thousands of individual primary human immune system cells. Perturbing these cells with molecular interventions drove the ordering of connections between pathway components, wherein Bayesian network computational methods automatically elucidated most of the traditionally reported signaling relationships and predicted novel interpathway network causalities, which we verified experimentally. Reconstruction of network models from physiologically relevant primary single cells might be applied to understanding native-state tissue signaling biology, complex drug actions, and dysfunctional signaling in diseased cells.}},
    author = {Sachs, Karen and Perez, Omar and Peer, Dana and Lauffenburger, Douglas A. and Nolan, Garry P.},
    citeulike-article-id = {257225},
    citeulike-linkout-0 = {http://dx.doi.org/10.1126/science.1105809},
    citeulike-linkout-1 = {http://www.sciencemag.org/content/308/5721/523.abstract},
    citeulike-linkout-2 = {http://www.sciencemag.org/content/308/5721/523.full.pdf},
    citeulike-linkout-3 = {http://www.sciencemag.org/cgi/content/abstract/308/5721/523},
    citeulike-linkout-4 = {http://view.ncbi.nlm.nih.gov/pubmed/15845847},
    citeulike-linkout-5 = {http://www.hubmed.org/display.cgi?uids=15845847},
    citeulike-linkout-6 = {http://www.sciencemag.org/cgi/content/full/308/5721/523},
    day = {22},
    doi = {10.1126/science.1105809},
    issn = {1095-9203},
    journal = {Science},
    keywords = {bayesian\_network},
    month = apr,
    number = {5721},
    pages = {523--529},
    pmid = {15845847},
    posted-at = {2010-03-19 20:19:43},
    priority = {2},
    title = {{Causal Protein-Signaling Networks Derived from Multiparameter Single-Cell Data}},
    url = {http://dx.doi.org/10.1126/science.1105809},
    volume = {308},
    year = {2005}
}



@article{rdfs,
    abstract = {{BACKGROUND: The recent availability of high-throughput data in molecular biology has increased the need for a formal representation of this knowledge domain. New ontologies are being developed to formalize knowledge, e.g. about the functions of proteins. As the Semantic Web is being introduced into the Life Sciences, the basis for a distributed knowledge-base that can foster biological data analysis is laid. However, there still is a dichotomy, in tools and methodologies, between the use of ontologies in biological investigation, that is, in relation to experimental observations, and their use as a knowledge-base. RESULTS: RDFScape is a plugin that has been developed to extend a software oriented to biological analysis with support for reasoning on ontologies in the semantic web framework. We show with this plugin how the use of ontological knowledge in biological analysis can be extended through the use of inference. In particular, we present two examples relative to ontologies representing biological pathways: we demonstrate how these can be abstracted and visualized as interaction networks, and how reasoning on causal dependencies within elements of pathways can be implemented. CONCLUSIONS: The use of ontologies for the interpretation of high-throughput biological data can be improved through the use of inference. This allows the use of ontologies not only as annotations, but as a knowledge-base from which new information relevant for specific analysis can be derived.}},
    address = {UPRES-EA 3888-Laboratoire d'Informatique M\'{e}dicale, Facult\'{e} de M\'{e}decine, Universit\'{e} Rennes 1, Rennes FR-35043, France. andrea.splendiani@univ-rennes1.fr},
    author = {Splendiani, Andrea},
    citeulike-article-id = {2784627},
    citeulike-linkout-0 = {http://dx.doi.org/10.1186/1471-2105-9-S4-S6},
    citeulike-linkout-1 = {http://view.ncbi.nlm.nih.gov/pubmed/18460179},
    citeulike-linkout-2 = {http://www.hubmed.org/display.cgi?uids=18460179},
    doi = {10.1186/1471-2105-9-S4-S6},
    issn = {1471-2105},
    journal = {BMC bioinformatics},
    keywords = {cytoscape, plugin},
    pmid = {18460179},
    posted-at = {2010-11-08 21:21:03},
    priority = {2},
    title = {{RDFScape: Semantic Web meets systems biology.}},
    url = {http://dx.doi.org/10.1186/1471-2105-9-S4-S6},
    volume = {9 Suppl 4},
    year = {2008}
}




@article{fages,
    abstract = {{The algorithms described in this article are implemented in the open-source software modeling platform BIOCHAM available at http://contraintes.inria.fr/biocham The models used in the experiments are available from http://www.biomodels.net/.}},
    author = {Gay, Steven and Soliman, Sylvain and Fages, Fran\c{c}ois},
    citeulike-article-id = {7796214},
    citeulike-linkout-0 = {http://dx.doi.org/10.1093/bioinformatics/btq388},
    citeulike-linkout-1 = {http://bioinformatics.oxfordjournals.org/content/26/18/i575.abstract},
    citeulike-linkout-2 = {http://bioinformatics.oxfordjournals.org/content/26/18/i575.full.pdf},
    citeulike-linkout-3 = {http://view.ncbi.nlm.nih.gov/pubmed/20823324},
    citeulike-linkout-4 = {http://www.hubmed.org/display.cgi?uids=20823324},
    day = {15},
    doi = {10.1093/bioinformatics/btq388},
    issn = {1367-4811},
    journal = {Bioinformatics (Oxford, England)},
    keywords = {networks},
    month = sep,
    number = {18},
    pages = {i575--i581},
    pmid = {20823324},
    posted-at = {2010-09-07 22:05:57},
    priority = {2},
    title = {{A graphical method for reducing and relating models in systems biology.}},
    url = {http://dx.doi.org/10.1093/bioinformatics/btq388},
    volume = {26},
    year = {2010}
}



@article{standards,
    abstract = {{High-throughput technologies are generating large amounts of complex data that have to be stored in databases, communicated to various data analysis tools and interpreted by scientists. Data representation and communication standards are needed to implement these steps efficiently. Here we give a classification of various standards related to systems biology and discuss various aspects of standardization in life sciences in general. Why are some standards more successful than others, what are the prerequisites for a standard to succeed and what are the possible pitfalls?}},
    author = {Brazma, Alvis and Krestyaninova, Maria and Sarkans, Ugis},
    citeulike-article-id = {763177},
    citeulike-linkout-0 = {http://dx.doi.org/10.1038/nrg1922},
    citeulike-linkout-1 = {http://dx.doi.org/10.1038/nrg1922},
    citeulike-linkout-2 = {http://view.ncbi.nlm.nih.gov/pubmed/16847461},
    citeulike-linkout-3 = {http://www.hubmed.org/display.cgi?uids=16847461},
    day = {01},
    doi = {10.1038/nrg1922},
    issn = {1471-0056},
    journal = {Nature Reviews Genetics},
    keywords = {systems\_biology},
    month = aug,
    number = {8},
    pages = {593--605},
    pmid = {16847461},
    posted-at = {2006-07-18 16:21:20},
    priority = {2},
    publisher = {Nature Publishing Group},
    title = {{Standards for systems biology}},
    url = {http://dx.doi.org/10.1038/nrg1922},
    volume = {7},
    year = {2006}
}


@UNPUBLISHED{mathpaper,
  AUTHOR =       {T. Petrov and A. Ganguly and H. Koeppl},
  TITLE =        {Markov chain aggregation and its applications to combinatorial reaction networks},
  NOTE =         {{}BISON group, ETH Zurich},
  year =         {in preparation},
}

@article{Peng1996b,
  added-at = {2008-04-23T22:05:04.000+0200},
  author = {Peng, Nan-Fu},
  biburl = {http://www.bibsonomy.org/bibtex/27a9919ad324c8c2cb8dd6b16e6af526e/smicha},
  day = 01,
  interhash = {d295d4238e318ed14a22b59b43f2aafe},
  intrahash = {7a9919ad324c8c2cb8dd6b16e6af526e},
  journal = {Statistics \& Probability Letters},
  keywords = {Markov chain},
  month = May,
  number = 4,
  pages = {313--318},
  timestamp = {2008-04-23T22:05:04.000+0200},
  title = {On weak lumpability of a finite Markov chain},
  url = {http://www.sciencedirect.com/science/article/B6V1D-3VSNHHN-N/1/769b18cd5a8669a132413b9296743b01},
  volume = 27,
  year = 1996
}



@ARTICLE{Philippe96numericalmethods,
    author = {Bernard Philippe and Youcef Saad and William J. Stewart},
    title = {Numerical Methods in Markov Chain Modelling},
    journal = {Operations Research},
    year = {1996},
    volume = {40},
    pages = {1156--1179}
}

@article{optimalKL,
  author    = {Kun Deng and
               Prashant G. Mehta and
               Sean P. Meyn},
  title     = {Optimal Kullback-Leibler Aggregation via Spectral Theory
               of Markov Chains},
  journal   = {IEEE Trans. Automat. Contr.},
  volume    = {56},
  number    = {12},
  year      = {2011},
  pages     = {2793-2808},
  ee        = {http://dx.doi.org/10.1109/TAC.2011.2141350},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}

@article{ramanujan18,
  author    = {Hardy and Ramanujan},
  title     = {Asymptotic Formula in Combinatory Analysis},
  journal   = {Proceedings of the London Mathematical Society},
  volume    = {S2-17(1)},
  year      = {1918},
  pages     = {75-115},
}

@inproceedings{lumpability,
  author = {Feret, Jerome and Henzinger, Thomas A. and Koeppl, Heinz and Petrov, Tatjana},
  editor = {Ciobanu, Gabriel and Koutny, Maciej},
  booktitle = {MeCBIC},
  crossref = {journals/corr/abs-1011-0051},
  interhash = {cad24c93c53e0f0e09de25011eec99ad},
  intrahash = {62aecfa23c8b55a854ee064160cb6656},
  pages = {142-161},
  series = {EPTCS},
  title = {Lumpability Abstractions of Rule-based Systems},
  url = {http://dblp.uni-trier.de/db/series/eptcs/eptcs40.html#abs-1011-0496},
  volume = 40,
  year = 2010,
  timestamp = {2010-12-15T00:00:00.000+0100},
  keywords = {dblp},
  ee = {http://dx.doi.org/10.4204/EPTCS.40.10},
  added-at = {2010-12-15T00:00:00.000+0100},
  biburl = {http://www.bibsonomy.org/bibtex/262aecfa23c8b55a854ee064160cb6656/dblp}
}




@article{conzelmann2008,
	Author = {Conzelmann, Holger and Fey, Dirk and Gilles, Ernst D.},
	Journal = {BMC Systems Biology},
	Number = {78},
	Pages = {342--351},
	Title = {Exact model reduction of combinatorial reaction networks},
	Volume = {2},
	Year = {2008}}


@article{2005PaulssonReview,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2005PhLRv...2..157P},
	Author = {{Paulsson}, J.},
	Doi = {10.1016/j.plrev.2005.03.003},
	Journal = {Physics of Life Reviews},
	Month = jun,
	Pages = {157-175},
	Title = {{Models of stochastic gene expression}},
	Volume = 2,
	Year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1016/j.plrev.2005.03.003}}

@article{geneticSwitch,
	Author = {Loinger, Adiel and Lipshtat, Azi and Balaban, Nathalie Q. and Biham, Ofer},
	Doi = {10.1103/PhysRevE.75.021904},
	Journal = {Phys. Rev. E},
	Month = {Feb},
	Number = {2},
	Numpages = {14},
	Pages = {021904},
	Publisher = {American Physical Society},
	Title = {Stochastic simulations of genetic switch systems},
	Volume = {75},
	Year = {2007},
	Bdsk-Url-1 = {http://dx.doi.org/10.1103/PhysRevE.75.021904}}

@techreport{Anderson2010,
	Author = {Anderson, David and Kurtz, Thomas G.},
	Citeulike-Article-Id = {8795016},
	Date-Added = {2011-03-03 14:28:06 +0100},
	Date-Modified = {2011-03-03 14:28:06 +0100},
	Institution = {University of Wisconsin - Madison},
	Keywords = {ctmc, modeling, simulation, stochastic\_simulation},
	Month = jul,
	Posted-At = {2011-02-09 21:13:33},
	Priority = {2},
	Title = {Continuous-time {M}arkov chain models for chemical reaction networks},
	Year = {2010}}

@article{verenaHybrid,
	Author = {Thomas A. Henzinger and Maria Mateescu and Linar Mikeev and Verena Wolf},
	Date-Added = {2010-12-05 21:49:33 -0500},
	Date-Modified = {2010-12-05 21:51:24 -0500},
	Journal = {CoRR},
	Rss-Description = {@article{DBLP:journals/corr/abs-1005-0747,
  author    = {Thomas A. Henzinger and Maria Mateescu and Linar Mikeev and Verena Wolf},
  title     = {Hybrid Numerical Solution of the Chemical Master Equation},
  journal   = {CoRR},
  volume    = {abs/1005.0747},
  year      = {2010},
  ee        = {http://arxiv.org/abs/1005.0747},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}},
	Title = {Hybrid Numerical Solution of the Chemical Master Equation},
	Year = {2010}}

@online{yeast2screening,
	Author = {Wikipedia},
	Month = jun,
	Title = {This is a test entry of type {@ONLINE}},
	Url = {http://en.wikipedia.org/wiki/Two-hybrid_screening},
	Year = {2010},
	Bdsk-Url-1 = {http://en.wikipedia.org/wiki/Two-hybrid_screening}}

@online{string,
	Author = {Wikipedia},
	Month = jun,
	Title = {This is a test entry of type {@ONLINE}},
	Url = {http://string-db.org/},
	Year = {2010},
	Bdsk-Url-1 = {http://string-db.org/}}

@article{sachs05,
	Abstract = {{Machine learning was applied for the automated derivation of causal influences in cellular signaling networks. This derivation relied on the simultaneous measurement of multiple phosphorylated protein and phospholipid components in thousands of individual primary human immune system cells. Perturbing these cells with molecular interventions drove the ordering of connections between pathway components, wherein Bayesian network computational methods automatically elucidated most of the traditionally reported signaling relationships and predicted novel interpathway network causalities, which we verified experimentally. Reconstruction of network models from physiologically relevant primary single cells might be applied to understanding native-state tissue signaling biology, complex drug actions, and dysfunctional signaling in diseased cells.}},
	Author = {Sachs, Karen and Perez, Omar and Pe'er, Dana and Lauffenburger, Douglas A. and Nolan, Garry P.},
	Citeulike-Article-Id = {257225},
	Citeulike-Linkout-0 = {http://dx.doi.org/10.1126/science.1105809},
	Citeulike-Linkout-1 = {http://www.sciencemag.org/content/308/5721/523.abstract},
	Citeulike-Linkout-2 = {http://www.sciencemag.org/content/308/5721/523.full.pdf},
	Citeulike-Linkout-3 = {http://www.sciencemag.org/cgi/content/abstract/308/5721/523},
	Citeulike-Linkout-4 = {http://view.ncbi.nlm.nih.gov/pubmed/15845847},
	Citeulike-Linkout-5 = {http://www.hubmed.org/display.cgi?uids=15845847},
	Citeulike-Linkout-6 = {http://www.sciencemag.org/cgi/content/full/308/5721/523},
	Day = {22},
	Doi = {10.1126/science.1105809},
	Issn = {1095-9203},
	Journal = {Science},
	Keywords = {bayesian\_network},
	Month = {April},
	Number = {5721},
	Pages = {523--529},
	Posted-At = {2010-03-19 20:19:43},
	Priority = {2},
	Title = {{Causal Protein-Signaling Networks Derived from Multiparameter Single-Cell Data}},
	Url = {http://dx.doi.org/10.1126/science.1105809},
	Volume = {308},
	Year = {2005},
	Bdsk-Url-1 = {http://dx.doi.org/10.1126/science.1105809}}

@article{Fagesmethod,
	Author = {Steven Gay, Sylvain Soliman and Fran{\c c}ois Fages},
	Date-Added = {2010-11-30 15:02:06 -0500},
	Date-Modified = {2010-11-30 15:02:06 -0500},
	Journal = {Bioinformatics 2010 26:i575-i581},
	Keywords = {European Conference on Computational Biology, ECCB'10},
	Read = {0},
	Rss-Description = {A Graphical Method for Reducing and Relating Models in Systems Biology by Steven Gay, Sylvain Soliman and Fran{\c c}ois Fages. European Conference on Computational Biology, ECCB'10, Ghent, Belgium. Bioinformatics 2010 26:i575-i581},
	Title = {A Graphical Method for Reducing and Relating Models in Systems Biology},
	Year = {2010}}

@article{kemperp_1996_1,
	Author = {Kemper, P.},
	Date-Added = {2010-08-03 14:49:26 +0200},
	Date-Modified = {2010-08-03 14:49:26 +0200},
	Journal = {IEEE T Software Eng},
	Number = {22},
	Pages = {615--628},
	Title = {Numerical Analysis of Superposed {GSPNs}},
	Volume = {9},
	Year = {1996}}

@article{journal,
	Author = {Jerome Feret and Heinz Koeppl and Tatjana Petrov},
	Date-Added = {2010-08-03 14:49:24 +0200},
	Date-Modified = {2010-08-03 14:49:24 +0200},
	Journal = {International Journal of Software and Informatics},
	Owner = {petrov},
	Title = {Stochastic fragments: A framework for the exact reduction of the stochastic semantics of rule-based models},
	Volume = {in press},
	Year = {2010}}

@inproceedings{sasb2011,
	Author = {Tatjana Petrov and Arnab Ganguly and Heinz Koeppl},
	Bibsource = {},
	Booktitle = {Proceedings of The Second International Workshop on Static Analysis and Systems Biology (SASB 2011)},
	Crossref = {},
	Date-Added = {},
	Date-Modified = {},
	Ee = {},
	Pages = {},
	Title = {Molecular Signaling-Model Decomposition and Stochastic Fragments},
	Year = {2011}}

@inproceedings{Donatelli94,
	Author = {Susanna Donatelli},
	Bibsource = {DBLP, http://dblp.uni-trier.de},
	Booktitle = {Application and Theory of Petri Nets},
	Crossref = {DBLP:conf/apn/1994},
	Date-Added = {2010-08-03 14:49:20 +0200},
	Date-Modified = {2010-08-03 14:49:20 +0200},
	Ee = {http://dx.doi.org/10.1007/3-540-58152-9_15},
	Pages = {258-277},
	Title = {Superposed Generalized Stochastic Petri Nets: Definition and Efficient Solution},
	Year = {1994}}

@inproceedings{Donatelli92,
	Author = {Susanna Donatelli and Matteo Sereno},
	Bibsource = {DBLP, http://dblp.uni-trier.de},
	Booktitle = {Application and Theory of Petri Nets},
	Crossref = {DBLP:conf/apn/1992},
	Date-Added = {2010-08-03 14:49:19 +0200},
	Date-Modified = {2010-08-03 14:49:19 +0200},
	Ee = {http://dx.doi.org/10.1007/3-540-55676-1_9},
	Pages = {154-172},
	Title = {On the Product Form Solution for Stochastic Petri Nets},
	Year = {1992}}

@article{conzelmann2006,
	Author = {Conzelmann, H. and Saez-Rodriguez, J. and Sauter, T. and Kholodenko, B. N. and Gilles, E. D.},
	Date-Added = {2010-08-03 14:49:18 +0200},
	Date-Modified = {2010-08-03 14:49:18 +0200},
	Journal = {BMC Syst Biol},
	Number = {34},
	Title = {A domain oriented approach to the reduction of combinatorial complexity in signal transduction networks},
	Volume = {7},
	Year = {2006}}

@article{changeux_2005_1,
	Author = {Changeux, J-P. and Edelstein, S. J.},
	Date-Added = {2010-08-03 14:49:16 +0200},
	Date-Modified = {2010-08-03 14:49:16 +0200},
	Journal = {Science},
	Pages = {1424--1428},
	Title = {Allosteric Mechanisms of Signal Transduction},
	Volume = {308},
	Year = {2005}}

@inproceedings{buchholzp_2004_1,
	Author = {Buchholz, P. and Kemper, P.},
	Booktitle = {Validation of Stochastic Systems},
	Date-Added = {2010-08-03 14:49:15 +0200},
	Date-Modified = {2010-08-03 14:49:15 +0200},
	Pages = {256---295},
	Series = {Lecture Notes in Computer Science},
	Title = {{Kronecker} Based Matrix Representations for Large {Markov} Models},
	Volume = {2925},
	Year = {2004}}

@article{buchholzp_2003_1,
	Author = {Buchholz, P. and Katoen, J-P. and Kemper, P. and Tepper, C.},
	Date-Added = {2010-08-03 14:49:14 +0200},
	Date-Modified = {2010-08-03 14:49:14 +0200},
	Journal = {Journal of Logic and Algebraic Programming},
	Number = {1-2},
	Pages = {69--97},
	Title = {Model-checking large structured {Markov} chains},
	Volume = {56},
	Year = {2003}}

@article{brewerj_1978_1,
	Author = {Brewer, J.},
	Date-Added = {2010-08-03 14:49:13 +0200},
	Date-Modified = {2010-08-03 14:49:13 +0200},
	Journal = {{IEEE} Transactions on Circuits and Systems},
	Keywords = {mathematics, nonlinear},
	Number = {9},
	Pages = {772--781},
	Title = {Kronecker products and matrix calculus in system theory},
	Volume = {25},
	Year = {1978}}

@article{borisovnm_2006_1,
	Author = {Borisov, N. M. and Markevich, N. I. and Hoek, J. B. and Kholodenko, B. N.},
	Date-Added = {2010-08-03 14:49:12 +0200},
	Date-Modified = {2010-08-03 14:49:12 +0200},
	Journal = {BioSystems},
	Pages = {152--166},
	Title = {Trading the micro-world of combinatorial complexity for the macro-world of protein interaction domains},
	Volume = {83},
	Year = {2006}}

@article{borisovnm_2005_1,
	Author = {Borisov, N. M. and Markevich, N. I. and Hoek, J. B. and Kholodenko, B. N.},
	Date-Added = {2010-08-03 14:49:11 +0200},
	Date-Modified = {2010-08-03 14:49:11 +0200},
	Journal = {Biophys J},
	Pages = {951---966},
	Title = {Signaling through Receptors and Scaffolds: Independent Interactions Reduce Combinatorial Complexity},
	Volume = {89},
	Year = {2005}}

@inproceedings{VerenaSW,
	Author = {Thomas A. Henzinger and Maria Mateescu and Verena Wolf},
	Bibsource = {DBLP, http://dblp.uni-trier.de},
	Booktitle = {CAV},
	Date-Added = {2010-08-03 14:49:04 +0200},
	Date-Modified = {2010-08-03 14:49:04 +0200},
	Pages = {337-352},
	Title = {Sliding Window Abstraction for Infinite {Markov} Chains},
	Year = {2009}}

@article{Verena2007StAut,
	Address = {Amsterdam, The Netherlands, The Netherlands},
	Author = {Wolf, Verena},
	Date-Added = {2010-08-03 14:49:03 +0200},
	Date-Modified = {2010-08-03 14:49:03 +0200},
	Doi = {http://dx.doi.org/10.1016/j.entcs.2007.05.017},
	Issn = {1571-0661},
	Journal = {Electron. Notes Theor. Comput. Sci.},
	Number = {2},
	Pages = {197--208},
	Publisher = {Elsevier Science Publishers B. V.},
	Title = {Modelling of Biochemical Reactions by Stochastic Automata Networks},
	Volume = {171},
	Year = {2007},
	Bdsk-Url-1 = {http://dx.doi.org/10.1016/j.entcs.2007.05.017}}

@article{vanZon2007,
	Author = {van Zon, Jeroen S. and Lubensky, David K. and Altena, Pim R. H. and Rein ten Wolde, Pieter},
	Date-Added = {2010-08-03 14:49:03 +0200},
	Date-Modified = {2010-08-03 14:49:03 +0200},
	Journal = {Proc Natl Acad Sci USA},
	Number = {18},
	Pages = {7420-7425},
	Title = {An allosteric model of circadian {KaiC} phosphorylation},
	Volume = {104},
	Year = {2007}}

@article{vanloancf_2000_1,
	Author = {Van Loan, C. F.},
	Date-Added = {2010-08-03 14:49:01 +0200},
	Date-Modified = {2010-08-03 14:49:01 +0200},
	Journal = {Comput Appl Math},
	Keywords = {mathematics},
	Pages = {85--100},
	Title = {The Ubiquitous Kronecker Product},
	Volume = {123},
	Year = {2000}}

@article{salazarc_2009_1,
	Author = {Carlos Salazar and Thomas H\"ofer},
	Date-Added = {2010-08-03 14:48:56 +0200},
	Date-Modified = {2010-08-03 14:48:56 +0200},
	Journal = {FEBS J},
	Pages = {3177--3198},
	Title = {Multisite protein phosphorylation - from molecular mechanisms to kinetic models},
	Volume = {276},
	Year = {2009}}

@inproceedings{plateaub_1985_1,
	Author = {Plateau, B.},
	Booktitle = {ACM SIGMETRICS Performance Evaluation Review},
	Date-Added = {2010-08-03 14:48:55 +0200},
	Date-Modified = {2010-08-03 14:48:55 +0200},
	Issue = {2},
	Pages = {147--154},
	Title = {On the stochastic structure of parallelism and synchronization models for distributed algorithms},
	Volume = {13},
	Year = {1985}}

@article{Nishiwaki2007,
	Author = {Nishiwaki, Taeko and Satomi, Yoshinori and Kitayama, Yohko and Terauchi, Kazuki and Kiyohara, Reiko and Takao, Toshifumi and Kondo, Takao},
	Date-Added = {2010-08-03 14:48:54 +0200},
	Date-Modified = {2010-08-03 14:48:54 +0200},
	Journal = {EMBO J},
	Number = {17},
	Pages = {4029-4037},
	Title = {A sequential program of dual phosphorylation of {KaiC} as a basis for circadian rhythm in cyanobacteria},
	Volume = {26},
	Year = {2007}}

@article{Nakajima2005,
	Author = {Nakajima, Masato and Imai, Keiko and Ito, Hiroshi and Nishiwaki, Taeko and Murayama, Yoriko and Iwasaki, Hideo and Oyama, Tokitaka and Kondo, Takao},
	Date-Added = {2010-08-03 14:48:53 +0200},
	Date-Modified = {2010-08-03 14:48:53 +0200},
	Journal = {Science},
	Pages = {414-415},
	Title = {Reconstitution of Circadian Oscillation of Cyanobacterial {KaiC} Phosphorylation in Vitro},
	Volume = {308},
	Year = {2005}}

@article{Mori2007,
	Author = {Tetsuya Mori and Dewight R. Willams and Mark O. Bryne and Ximing Qin and Martin Egli and Hassane S. Mchaourab and Phoebe L. Stewart and Carl H. Johnson},
	Date-Added = {2010-08-03 14:48:52 +0200},
	Date-Modified = {2010-08-03 14:48:52 +0200},
	Journal = {PLoS Biol},
	Number = {4},
	Pages = {841-853},
	Title = {Elucidating the Ticking of an In Vitro Circadian Clockwork},
	Volume = {5},
	Year = {2007}}

@article{weakLumpDTMC,
	Abstract = {cannot paste it},
	Author = {Gerardo Rubino and Bruno Sericola},
	Date-Added = {2010-08-03 14:48:30 +0200},
	Date-Modified = {2010-08-03 14:48:30 +0200},
	Journal = {Stochastic processes and their applications},
	Owner = {petrov},
	Pages = {115-125},
	Review = {Characterization and a finite algorithm of weak/strong/exact lumpability},
	Timestamp = {2010.01.15},
	Title = {A Finite Characterization of Weak Lumpable {Markov} Processes. Part {I}: The Discrete Time Case},
	Volume = {vol. 45, no 1},
	Year = {1993}}

@article{weakLumpCTMC,
	Abstract = {cannot paste it},
	Author = {Gerardo Rubino and Bruno Sericola},
	Date-Added = {2010-08-03 14:48:29 +0200},
	Date-Modified = {2010-08-03 14:48:29 +0200},
	Journal = {Stochastic processes and their applications},
	Owner = {petrov},
	Pages = {195-204},
	Review = {An algorithmic characterization of weak lumpability on a CTMC},
	Timestamp = {2010.01.15},
	Title = {A Finite Characterization of Weak Lumpable {Markov Processes}. Part {II}: The Continuous Time Case},
	Volume = {vol. 38, no2},
	Year = {1991}}

@article{unif2,
	Abstract = {The uniformization method (also known as randomization) is a numerically
	stable algorithm for computing transient distributions of a continuous
	time Markov chain. When the solution is needed after a long run or
	when the convergence is slow, the uniformization method involves
	a large number of matrix-vector products. Despite this, the method
	remains very popular due to its ease of implementation and its reliability
	in many practical circumstances. Because calculating the matrix-vector
	product is the most time-consuming part of the method, overall efficiency
	in solving large-scale problems can be significantly enhanced if
	the matrix-vector product is made more economical. In this paper,
	we incorporate a new relaxation strategy into the uniformization
	method to compute the matrix-vector products only approximately.
	We analyze the error introduced by these inexact matrix-vector products
	and discuss strategies for refining the accuracy of the relaxation
	while reducing the execution cost. Numerical experiments drawn from
	computer systems and biological systems are given to show that significant
	computational savings are achieved in practical applications.},
	Author = {Roger B. Sidje, Kevin Burrage, and Shev MacNamara},
	Date-Added = {2010-08-03 14:48:27 +0200},
	Date-Modified = {2010-08-03 14:48:27 +0200},
	Journal = {SIAM Journal on Scientific Computing},
	Owner = {petrov},
	Pages = {2562-2580},
	Review = {unofrmization...},
	Timestamp = {2010.01.15},
	Title = {Inexact Uniformization Method for Computing Transient Distributions of {Markov} Chains},
	Volume = {29, issue 6},
	Year = {2007}}

@article{unif1,
	Abstract = {We present a randomization procedure for computing transient solutions
	to discrete state space, continuous time Markov processes. This procedure
	computes transient state probabilities. It is based on a construction
	relating a continuous time Markov process to a discrete time Markov
	chain. Modifications and extensions of the randomization method allow
	for computation of distributions of first passage times and sojourn
	times in Markov processes, and also the computation of expected cumulative
	occupancy times and expected number of events occurring during a
	time interval. Several implementations of the randomization procedure
	are discussed. In particular we present an implementation for a general
	class of Markov processes that can be described in terms of state
	space (S), event set (E), rate vectors (R), and target vectors (T)�abbreviated
	as SERT. This general approach can handle systems whose state spaces
	are quite large, if they have sparse generators.},
	Author = {Donald Gross and Douglas R. Miller},
	Date-Added = {2010-08-03 14:48:27 +0200},
	Date-Modified = {2010-08-03 14:48:27 +0200},
	Journal = {Operations Research},
	Owner = {petrov},
	Pages = {343-361},
	Review = {uniformization of a CTMC},
	Timestamp = {2010.01.15},
	Title = {The Randomization Technique as a Modeling Tool and Solution Procedure for Transient {Markov} Processes},
	Volume = {32, no2},
	Year = {1984}}

@inproceedings{susanna,
	Address = {Washington, DC, USA},
	Author = {Sproston, Jeremy and Donatelli, Susanna},
	Booktitle = {QEST '04},
	Date-Added = {2010-08-03 14:48:26 +0200},
	Date-Modified = {2010-08-03 14:48:26 +0200},
	Doi = {http://dx.doi.org/10.1109/QEST.2004.10},
	Isbn = {0-7695-2185-1},
	Pages = {220--229},
	Title = {Backward Stochastic Bisimulation in {CSL} Model Checking},
	Year = {2004},
	Bdsk-Url-1 = {http://dx.doi.org/10.1109/QEST.2004.10}}

@inproceedings{Sokolova03onrelational,
	Author = {Ana Sokolova and Vink, Erik P. de},
	Booktitle = {Proceedings of the 4th PROGRESS},
	Date-Added = {2010-08-03 14:48:24 +0200},
	Date-Modified = {2010-08-03 14:48:24 +0200},
	Title = {On relational properties of lumpability},
	Year = 2003}

@article{smockr_2009_1,
	Author = {Robert G. Smock and Lila M. Gierasch},
	Date-Added = {2010-08-03 14:48:23 +0200},
	Date-Modified = {2010-08-03 14:48:23 +0200},
	Journal = {Science},
	Pages = {198--203},
	Title = {Sending signals dynamically},
	Volume = {324},
	Year = {2009}}

@misc{SI,
	Author = {Jerome Feret and Thomas Henzinger and Heinz Koeppl and Tatjana Petrov},
	Date-Added = {2010-08-03 14:48:22 +0200},
	Date-Modified = {2010-08-03 14:48:22 +0200},
	Title = {Supporting information under {http://lanos.epfl.ch/sysbio/CMSB2010Supp.pdf}},
	Url = {http://lanos.epfl.ch/sysbio/CMSB2010_Supp.pdf},
	Year = {2010},
	Bdsk-Url-1 = {http://lanos.epfl.ch/sysbio/CMSB2010_Supp.pdf}}

@article{kurtztg_1971_1,
	Author = {Thomas G. Kurtz},
	Date-Added = {2010-08-03 14:48:13 +0200},
	Date-Modified = {2010-08-03 14:48:13 +0200},
	Journal = {Journal of Applied Probability},
	Number = {2},
	Pages = {344--356},
	Title = {Limit Theorems for Sequences of Jump {Markov} Processes Approximating Ordinary Differential Processes},
	Volume = {8},
	Year = {1971}}

@book{kemeny1976,
	Address = {New York, NY, USA},
	Author = {Kemeny, J. G. and Snell, J. L. and Knapp, A. W.},
	Date-Added = {2010-08-03 14:48:12 +0200},
	Date-Modified = {2010-08-03 14:48:12 +0200},
	Isbn = {0-521-57189-8},
	Publisher = {Springer-Verlag},
	Title = {Denumerable {M}arkov Chains},
	Year = {1976}}

@inproceedings{jean,
	Author = {Jean Krivine and Robin Milner and Angelo Troina},
	Booktitle = {Proceedings of the 24th Conference on the Mathematical Foundations of Programming Semantics (MFPS XXIV)},
	Date-Added = {2010-08-03 14:48:11 +0200},
	Date-Modified = {2010-08-03 14:48:11 +0200},
	Pages = {73--96},
	Series = {ENTCS},
	Title = {Stochastic Bigraphs},
	Volume = {218},
	Year = {2008}}

@book{janePhD,
	Address = {New York, NY, USA},
	Author = {Hillston, Jane},
	Date-Added = {2010-08-03 14:48:10 +0200},
	Date-Modified = {2010-08-03 14:48:10 +0200},
	Isbn = {0-521-57189-8},
	Publisher = {Cambridge University Press},
	Title = {A compositional approach to performance modelling},
	Year = {1996}}

@inproceedings{jane,
	Author = {Jane Hilston},
	Booktitle = {Second International Workshop on Numerical Solution of Markov Chains: Computations with Markov Chains, Kluwer Academic Press},
	Date-Added = {2010-08-03 14:48:09 +0200},
	Date-Modified = {2010-08-03 14:48:09 +0200},
	Title = {Compositional {Markovian} Modelling Using A Process Algebra},
	Year = {January 1995}}

@inproceedings{danos:aplas07,
	Address = {Singapore},
	Author = {V.\ Danos and J.\ Feret and W.\ Fontana and J.\ Krivine},
	Booktitle = {Proceedings of the Fifth Asian Symposium on Programming Systems, APLAS$\,$'2007, Singapore},
	Date-Added = {2010-08-03 14:48:01 +0200},
	Date-Modified = {2010-08-03 14:48:01 +0200},
	Editor = {Z.\ Shao},
	Month = {29 November -- 1 December},
	Pages = {139--157},
	Publisher = {Springer, Berlin, Germany},
	Series = {Lecture Notes in Computer Science},
	Title = {Scalable Simulation of Cellular Signaling Networks, invited paper},
	Volume = {4807},
	Year = {2007}}

@article{buchholz_lump,
	Abstract = {Exact and ordinary lumpability in finite Markov chains is considered.
	Both concepts naturally define an aggregation of the Markov chain
	yielding an},
	Author = {Peter Buchholz},
	Date-Added = {2010-08-03 14:48:00 +0200},
	Date-Modified = {2010-08-03 14:48:00 +0200},
	Journal = {Journal of Applied Probability},
	Owner = {petrov},
	Pages = {59-75},
	Timestamp = {2010.01.15},
	Title = {Exact and Ordinary Lumpability in Finite {Markov} Chains},
	Volume = {31, no1},
	Year = {1994}}

@article{buchholz_bisimulation,
	Abstract = {Bisimulation is a well known equivalence relation for discrete event
	systems and has been extended to probabilistic and stochastic systems.
	This paper introduces a general definition of bisimulation which
	can be applied to finite automata where weights and labels are assigned
	to transitions. It is shown that this general view contains several
	known bisimulations as special cases and defines naturally equivalences
	for different classes of models. Apart from the well known forward
	bisimulation, also backward bisimulation is introduced and it is
	shown that both types of bisimulation preserve different types of
	results. Furthermore it is shown that forward and backward bisimulation
	are congruences according to commonly known composition operations
	for automata.},
	Author = {Peter Buchholz},
	Date-Added = {2010-08-03 14:47:59 +0200},
	Date-Modified = {2010-08-03 14:47:59 +0200},
	Journal = {Theoretical Computer Science},
	Owner = {petrov},
	Pages = {109-123},
	Timestamp = {2010.01.15},
	Title = {Bisimulation relations for weighted automata},
	Volume = {Volume 393, Issue 1-3},
	Year = {2008}}

@article{baier03,
	Author = {Christel Baier and Boudewijn Haverkort and Holger Hermanns and Joost-Pieter Katoen},
	Date-Added = {2010-08-03 14:47:58 +0200},
	Date-Modified = {2010-08-03 14:47:58 +0200},
	Journal = {IEEE Transactions on Software Engineering},
	Number = {7},
	Pages = {2003},
	Title = {Model-checking algorithms for continuous-time {Markov} chains},
	Volume = {29},
	Year = {2003}}

@phdthesis{holger_PhD,
	Abstract = {Interactive Markov Chains
	
	And the Quest for Quantified Quality
	
	Book Series	Lecture Notes in Computer Science
	
	Publisher	Springer Berlin / Heidelberg
	
	ISSN	0302-9743 (Print) 1611-3349 (Online)
	
	Volume	Volume 2428/2002
	
	DOI	10.1007/3-540-45804-2
	
	Copyright	2002
	
	ISBN	978-3-540-44261-5
	
	Subject Collection	Computer Science
	
	SpringerLink Date	Saturday, August 02, 2003},
	Author = {Holger Hermanns},
	Date-Added = {2010-08-03 14:47:51 +0200},
	Date-Modified = {2010-08-03 14:47:51 +0200},
	Owner = {petrov},
	School = {University of Marburg},
	Timestamp = {2010.01.15},
	Title = {Interactive {Markov} Chains And the Quest for Quantified Quality},
	Year = {2002}}

@article{kurtztg_1970_1,
	Author = {Thomas G. Kurtz},
	Date-Added = {2010-08-03 14:47:50 +0200},
	Date-Modified = {2010-08-03 14:47:50 +0200},
	Journal = {Journal of Applied Probability},
	Number = {1},
	Pages = {49--58},
	Title = {Solutions of Ordinary Differential Equations as Limits of Pure Jump {Markov} Processes},
	Volume = {7},
	Year = {1970}}

@article{lumpCommutCTMCExact,
	Abstract = {We introduce the concepts of lumpability and commutativity of a continuous
	time discrete state space Markov process, and provide a necessary
	and sufficient condition for a lumpable Markov process to be commutative.
	Under suitable conditions we recover some of the basic quantities
	of the original Markov process from the jump chain of the lumped
	Markov process.},
	Author = {Jianjun Paul Tian, D. Kannan},
	Date-Added = {2010-08-03 14:47:49 +0200},
	Date-Modified = {2010-08-03 14:47:49 +0200},
	Journal = {Stochastic analysis and Applications},
	Owner = {petrov},
	Pages = {685-702},
	Timestamp = {2010.01.15},
	Title = {Lumpability and Commutativity of {Markov} Processes},
	Volume = {24, no3},
	Year = {2006}}

@article{PengWeak,
	Abstract = {An irreducible and homogeneous Markov chain with finite state space is considered. Under a mild condition [Gamma] on the transition probability matrix, a necessary and sufficient condition for weak lumpability, and the characterization of the set of initial starting vectors which make it lumpable are obtained. A similar result is obtained for those transition probability matrices without the restriction of condition [Gamma].},
	Author = {Peng, Nan-Fu},
	Date-Added = {2010-08-03 14:47:48 +0200},
	Date-Modified = {2010-08-03 14:47:48 +0200},
	Journal = {Statistics \& Probability Letters},
	Keywords = {Markov chain Weak lumpability},
	Month = {May},
	Number = {4},
	Pages = {313-318},
	Title = {On weak lumpability of a finite {Markov} chain},
	Url = {http://ideas.repec.org/a/eee/stapro/v27y1996i4p313-318.html},
	Volume = {27},
	Year = 1996,
	Bdsk-Url-1 = {http://ideas.repec.org/a/eee/stapro/v27y1996i4p313-318.html}}

@article{Webster2009,
	Author = {Gordon Webster},
	Citeulike-Article-Id = {4709732},
	Date-Added = {2010-08-03 14:47:17 +0200},
	Date-Modified = {2010-08-03 14:47:17 +0200},
	Journal = {Drug Discovery World},
	Posted-At = {2009-06-01 18:00:38},
	Priority = {2},
	Title = {Biologists flirt with models},
	Year = {2009}}

@article{vardi99probabilistic,
	Author = {Moshe Y. Vardi},
	Date-Added = {2010-08-03 14:47:16 +0200},
	Date-Modified = {2010-08-03 14:47:16 +0200},
	Journal = {Lecture Notes in Computer Science},
	Pages = {265--276},
	Title = {Probabilistic Linear-Time Model Checking: An Overview of the Automata-Theoretic Approach},
	Url = {citeseer.ist.psu.edu/vardi99probabilistic.html},
	Volume = {1601},
	Year = {1999},
	Bdsk-Url-1 = {citeseer.ist.psu.edu/vardi99probabilistic.html}}

@book{StewartMC,
	Author = {William J. Stewart},
	Date-Added = {2010-08-03 14:47:16 +0200},
	Date-Modified = {2010-08-03 14:47:16 +0200},
	Publisher = {Princeton University Press},
	Title = {Introduction to the Numerical Solution of Markov Chains},
	Year = {2005}}

@article{Regev2,
	Address = {Essex, UK},
	Author = {Aviv Regev and Ekaterina M. Panina and Willam Silverman and Luca Cardelli and Ehud Shapiro},
	Date-Added = {2010-08-03 14:47:13 +0200},
	Date-Modified = {2010-08-03 14:50:36 +0200},
	Doi = {http://dx.doi.org/10.1016/j.tcs.2004.03.061},
	Issn = {0304-3975},
	Journal = {Theoretical Computer Science},
	Number = {1},
	Pages = {141--167},
	Publisher = {Elsevier Science Publishers Ltd.},
	Title = {BioAmbients: an abstraction for biological compartments},
	Volume = {325},
	Year = {2004},
	Bdsk-Url-1 = {http://dx.doi.org/10.1016/j.tcs.2004.03.061}}

@article{RB28,
	Abstract = {No abstract is available for this item.},
	Author = {John Haigh},
	Date-Added = {2010-08-03 14:47:12 +0200},
	Date-Modified = {2010-08-03 14:47:12 +0200},
	Journal = {Journal Of The Royal Statistical Society Series A},
	Number = {1},
	Pages = {261-261},
	Title = {Stochastic Modelling for Systems Biology by D. J. Wilkinson},
	Url = {http://ideas.repec.org/a/bla/jorssa/v170y2007i1p261-261.html},
	Volume = {170},
	Year = {2007},
	Bdsk-Url-1 = {http://ideas.repec.org/a/bla/jorssa/v170y2007i1p261-261.html}}

@article{RB27,
	Author = {T.W. Anderson and Leo A. Goodman},
	Citeulike-Article-Id = {2820303},
	Citeulike-Linkout-0 = {http://projecteuclid.org/euclid.aoms/1177707039},
	Date-Added = {2010-08-03 14:47:11 +0200},
	Date-Modified = {2010-08-03 14:47:11 +0200},
	Journal = {The Annals of Mathematical Statistics},
	Keywords = {markov-chains, statistics},
	Number = {1},
	Pages = {89-110},
	Posted-At = {2008-05-21 16:08:01},
	Priority = {2},
	Title = {Statistical Inference about Markov Chains},
	Url = {http://projecteuclid.org/euclid.aoms/1177707039},
	Volume = {28},
	Year = {1957},
	Bdsk-Url-1 = {http://projecteuclid.org/euclid.aoms/1177707039}}

@article{RB16,
	Abstract = {BioNetGen allows a user to create a computational model that characterizes
	the dynamics of a signal transduction system, and that accounts comprehensively
	and precisely for specified enzymatic activities, potential post-translational
	modifications and interactions of the domains of signaling molecules.
	The output defines and parameterizes the network of molecular species
	that can arise during signaling and provides functions that relate
	model variables to experimental readouts of interest. Models that
	can be generated are relevant for rational drug discovery, analysis
	of proteomic data and mechanistic studies of signal transduction.},
	Address = {Theoretical Biology and Biophysics Group, Theoretical Division, Los Alamos National Laboratory, Los Alamos, NM 87545, USA.},
	Author = {M. Blinov and J.R. Faeder and B. Goldstein and W.S. Hlavacek},
	Citeulike-Article-Id = {2839907},
	Citeulike-Linkout-0 = {http://view.ncbi.nlm.nih.gov/pubmed/15217809},
	Citeulike-Linkout-1 = {http://www.hubmed.org/display.cgi?uids=15217809},
	Date-Added = {2010-08-03 14:47:11 +0200},
	Date-Modified = {2010-08-03 14:47:11 +0200},
	Issn = {1367-4803},
	Journal = {Bioinformatics (Oxford, England)},
	Month = {November},
	Number = {17},
	Pages = {3289--3291},
	Posted-At = {2008-05-28 08:30:06},
	Priority = {2},
	Title = {BioNetGen: software for rule-based modeling of signal transduction based on the interactions of molecular domains.},
	Url = {http://view.ncbi.nlm.nih.gov/pubmed/15217809},
	Volume = {20},
	Year = {2004},
	Bdsk-Url-1 = {http://view.ncbi.nlm.nih.gov/pubmed/15217809}}

@article{RB15,
	Author = {L. Lok and R. Brent},
	Citeulike-Article-Id = {72880},
	Citeulike-Linkout-0 = {http://dx.doi.org/10.1038/nbt1054},
	Citeulike-Linkout-1 = {http://dx.doi.org/10.1038/nbt1054},
	Citeulike-Linkout-2 = {http://view.ncbi.nlm.nih.gov/pubmed/15637632},
	Citeulike-Linkout-3 = {http://www.hubmed.org/display.cgi?uids=15637632},
	Date-Added = {2010-08-03 14:47:09 +0200},
	Date-Modified = {2010-08-03 14:47:09 +0200},
	Doi = {10.1038/nbt1054},
	Issn = {1087-0156},
	Journal = {Nature Biotechnology},
	Keywords = {moleculizer, simulation},
	Month = {January},
	Number = {1},
	Pages = {131--136},
	Posted-At = {2009-01-13 06:11:34},
	Priority = {2},
	Publisher = {Nature Publishing Group},
	Title = {Automatic generation of cellular reaction networks with Moleculizer 1.0},
	Url = {http://dx.doi.org/10.1038/nbt1054},
	Volume = {23},
	Year = {2005},
	Bdsk-Url-1 = {http://dx.doi.org/10.1038/nbt1054}}

@article{RB14,
	Abstract = {We consider a model of early events in signaling by the epidermal
	growth factor (EGF) receptor (EGFR). The model includes EGF, EGFR,
	the adapter proteins Grb2 and Shc, and the guanine nucleotide exchange
	factor Sos, which is activated through EGF-induced formation of EGFR-Grb2-Sos
	and EGFR-Shc-Grb2-Sos assemblies at the plasma membrane. The protein
	interactions involved in signaling can potentially generate a diversity
	of protein complexes and phosphoforms; however, this diversity has
	been largely ignored in models of EGFR signaling. Here, we develop
	a model that accounts more fully for potential molecular diversity
	by specifying rules for protein interactions and then using these
	rules to generate a reaction network that includes all chemical species
	and reactions implied by the protein interactions. We obtain a model
	that predicts the dynamics of 356 molecular species, which are connected
	through 3749 unidirectional reactions. This network model is compared
	with a previously developed model that includes only 18 chemical
	species but incorporates the same scope of protein interactions.
	The predictions of this model are reproduced by the network model,
	which also yields new predictions. For example, the network model
	predicts distinct temporal patterns of autophosphorylation for different
	tyrosine residues of EGFR. A comparison of the two models suggests
	experiments that could lead to mechanistic insights about competition
	among adapter proteins for EGFR binding sites and the role of EGFR
	monomers in signal transduction.},
	Author = {M.L. Blinov},
	Date-Added = {2010-08-03 14:47:08 +0200},
	Date-Modified = {2010-08-03 14:47:08 +0200},
	Day = {17},
	Issn = {0303-2647},
	Journal = {Biosystems},
	Keywords = {Animals},
	Language = {eng},
	Month = {Feb/Mar},
	Number = {2-3},
	Pages = {136--151},
	Title = {A network model of early events in epidermal growth factor receptor signaling that accounts for combinatorial complexity.},
	Volume = {83},
	Year = {2006}}

@article{RB13,
	Abstract = {We describe a general approach to automatic model generation in the
	description of dynamic regulatory networks.},
	Author = {B.E. Shapiro and A. Levchenko and E. Mjolsness},
	Date-Added = {2010-08-03 14:47:07 +0200},
	Date-Modified = {2010-08-03 14:47:07 +0200},
	Journal = {First International Conference on Systems Biology},
	Keywords = {grn, indirect},
	Location = {Tokyo, Japan},
	Pages = {64-74},
	Posted-At = {2008-07-24 10:36:49},
	Priority = {2},
	Title = {Automatic model generation for signal transduction with applications to MAP-Kinase pathways},
	Url = {http://trs-new.jpl.nasa.gov/dspace/handle/2014/15876?mode=simple},
	Year = {2000},
	Bdsk-Url-1 = {http://trs-new.jpl.nasa.gov/dspace/handle/2014/15876?mode=simple}}

@inproceedings{RB11,
	Author = {Steven Eker and Merrill Knapp and Keith Laderoute and Patrick Lincoln and Jos\'{e} Meseguer and Kemal Sonmez},
	Booktitle = {Proceedings of the Pacific Symposium on Biocomputing},
	Date-Added = {2010-08-03 14:47:07 +0200},
	Date-Modified = {2010-08-03 14:47:07 +0200},
	Pages = {400-412},
	Title = {Pathway Logic: Symbolic Analysis of Biological Signaling},
	Url = {http://www.csl.sri.com/papers/lincoln-pathway-logic-psb-2002/},
	Year = {2002},
	Bdsk-Url-1 = {http://www.csl.sri.com/papers/lincoln-pathway-logic-psb-2002/}}

@inproceedings{RB10,
	Author = {Luca Cardelli},
	Date-Added = {2010-08-03 14:47:06 +0200},
	Date-Modified = {2010-08-03 14:47:06 +0200},
	Pages = {257--280},
	Publisher = {Springer},
	Title = {Brane Calculi, Interactions of Biological Membranes},
	Year = {2005}}

@article{RB09,
	Address = {Essex, UK},
	Author = {Vincent Danos and Cosimo Laneve},
	Date-Added = {2010-08-03 14:47:05 +0200},
	Date-Modified = {2010-08-03 14:47:05 +0200},
	Doi = {http://dx.doi.org/10.1016/j.tcs.2004.03.065},
	Issn = {0304-3975},
	Journal = {Theoretical Computer Science},
	Number = {1},
	Pages = {69--110},
	Publisher = {Elsevier Science Publishers Ltd.},
	Title = {Formal molecular biology},
	Volume = {325},
	Year = {2004},
	Bdsk-Url-1 = {http://dx.doi.org/10.1016/j.tcs.2004.03.065}}

@article{RB08,
	Author = {Vincent Danos and Jean Krivine},
	Bibsource = {DBLP, http://dblp.uni-trier.de},
	Date-Added = {2010-08-03 14:47:05 +0200},
	Date-Modified = {2010-08-03 14:47:05 +0200},
	Ee = {http://dx.doi.org/10.1016/j.entcs.2004.01.040},
	Journal = {Electronic Notes in Theoretical Computer Science},
	Number = {3},
	Pages = {31-49},
	Title = {Formal Molecular Biology Done in CCS-R},
	Volume = {180},
	Year = {2007}}

@article{RB4,
	Author = {W.S. Hlavacek},
	Date-Added = {2010-08-03 14:47:04 +0200},
	Date-Modified = {2010-08-03 14:47:04 +0200},
	Journal = {Biotechnology and Bio-engineering},
	Owner = {petrov},
	Pages = {783-794},
	Timestamp = {2009.07.01},
	Title = {The complexity of complexes in signal transduction},
	Volume = {84},
	Year = {2005}}

@article{RB3,
	Author = {C.T. Walsh},
	Date-Added = {2010-08-03 14:47:03 +0200},
	Date-Modified = {2010-08-03 14:47:03 +0200},
	Journal = {Roberts and Co. Publisher},
	Owner = {Tatjana},
	Timestamp = {2009.07.15},
	Title = {Posttranslational Modification of Proteins: Expanding Nature's Inventory},
	Year = {2006}}

@article{RB1,
	Abstract = {Formalized rules for protein-protein interactions have recently been
	introduced to represent the binding and enzymatic activities of proteins
	in cellular signaling. Rules encode an understanding of how a system
	works in terms of the biomolecules in the system and their possible
	states and interactions. A set of rules can be as easy to read as
	a diagrammatic interaction map, but unlike most such maps, rules
	have precise interpretations. Rules can be processed to automatically
	generate a mathematical or computational model for a system, which
	enables explanatory and predictive insights into the system's behavior.
	Rules are independent units of a model specification that facilitate
	model revision. Instead of changing a large number of equations or
	lines of code, as may be required in the case of a conventional mathematical
	model, a protein interaction can be introduced or modified simply
	by adding or changing a single rule that represents the interaction
	of interest. Rules can be defined and visualized by using graphs,
	so no specialized training in mathematics or computer science is
	necessary to create models or to take advantage of the representational
	precision of rules. Rules can be encoded in a machine-readable format
	to enable electronic storage and exchange of models, as well as basic
	knowledge about protein-protein interactions. Here, we review the
	motivation for rule-based modeling; applications of the approach;
	and issues that arise in model specification, simulation, and testing.
	We also discuss rule visualization and exchange and the software
	available for rule-based modeling.},
	Address = {Center for Nonlinear Studies, Los Alamos National Laboratory, Los Alamos, NM 87545, USA. wish@lanl.gov},
	Author = {W.S. Hlavacek and J.R. Faeder and M.L. Blinov and R.G. Posner and M. Hucka and W. Fontana},
	Citeulike-Article-Id = {984344},
	Citeulike-Linkout-0 = {http://dx.doi.org/10.1126/stke.3442006re6},
	Citeulike-Linkout-1 = {http://view.ncbi.nlm.nih.gov/pubmed/16849649},
	Citeulike-Linkout-2 = {http://www.hubmed.org/display.cgi?uids=16849649},
	Date-Added = {2010-08-03 14:47:03 +0200},
	Date-Modified = {2010-08-03 14:47:03 +0200},
	Doi = {10.1126/stke.3442006re6},
	Issn = {1525-8882},
	Journal = {Science's STKE},
	Keywords = {cellucidate, modeling, plectix, simulation},
	Month = {July},
	Number = {344},
	Posted-At = {2009-06-20 21:48:12},
	Priority = {2},
	Title = {Rules for modeling signal-transduction systems.},
	Url = {http://dx.doi.org/10.1126/stke.3442006re6},
	Year = {2006},
	Bdsk-Url-1 = {http://dx.doi.org/10.1126/stke.3442006re6}}

@article{RB-sim-1,
	Author = {Vincent Danos and Jerome Feret and Walter Fontana and Jean Krivine},
	Date-Added = {2010-08-03 14:47:01 +0200},
	Date-Modified = {2010-08-03 14:47:01 +0200},
	Journal = {In Proceedings of APLAS 2007},
	Owner = {petrov},
	Timestamp = {2009.07.01},
	Title = {Scalable simulation of cellular signaling networks},
	Year = {2007}}

@inproceedings{RB_CAVTutorial09,
	Author = {J. Krivine and V. Danos and A. Benecke},
	Bibsource = {DBLP, http://dblp.uni-trier.de},
	Booktitle = {CAV},
	Crossref = {DBLP:conf/cav/2009},
	Date-Added = {2010-08-03 14:47:00 +0200},
	Date-Modified = {2010-08-03 14:47:00 +0200},
	Ee = {http://dx.doi.org/10.1007/978-3-642-02658-4_3},
	Pages = {17-32},
	Title = {Modelling Epigenetic Information Maintenance: A Kappa Tutorial},
	Year = {2009}}

@article{probBisimulationPrakash,
	Author = {Desharnais, J. and Edalat, A. and Panangaden, P.},
	Citeulike-Article-Id = {53126},
	Citeulike-Linkout-0 = {http://dx.doi.org/10.1006/inco.2001.2962},
	Citeulike-Linkout-1 = {http://www.ingentaconnect.com/content/ap/ic/2002/00000179/00000002/art02962},
	Date-Added = {2010-08-03 14:46:58 +0200},
	Date-Modified = {2010-08-03 14:46:58 +0200},
	Doi = {10.1006/inco.2001.2962},
	Issn = {0890-5401},
	Journal = {Information and Computation},
	Month = {December},
	Number = {2},
	Pages = {163--193},
	Posted-At = {2004-12-28 17:51:32},
	Publisher = {Academic Press},
	Title = {Bisimulation for Labelled Markov Processes},
	Url = {http://dx.doi.org/10.1006/inco.2001.2962},
	Volume = {179},
	Year = {2002},
	Bdsk-Url-1 = {http://dx.doi.org/10.1006/inco.2001.2962}}

@article{TianCommutativity,
author = {Tian, Jianjun   Paul and Kannan, D.},
title = {Lumpability and Commutativity of Markov Processes},
journal = {Stochastic Analysis and Applications},
volume = {24},
number = {3},
pages = {685-702},
year = {2006},
doi = {10.1080/07362990600632045},

URL = {http://www.tandfonline.com/doi/abs/10.1080/07362990600632045},
eprint = {http://www.tandfonline.com/doi/pdf/10.1080/07362990600632045}
}



@article{ODEfragm2,
	Author = {Vincent Danos and Jerome Feret and Walter Fontana and Jean Krivine},
	Date-Added = {2010-08-03 14:46:57 +0200},
	Date-Modified = {2010-08-03 14:46:57 +0200},
	Keywords = {Rule-based, Abstract-Interpretation, deterministic semantics},
	Owner = {petrov},
	Timestamp = {2009.06.26},
	Title = {Abstracting the ODE Semantics of Rule-Based Models: Exact and Automatic Model Reduction},
	Year = {2009}}

@book{MilnerPi,
	Author = {Robin Milner},
	Date-Added = {2010-08-03 14:46:56 +0200},
	Date-Modified = {2010-08-03 14:46:56 +0200},
	Howpublished = {Paperback},
	Isbn = {0521658691},
	Keywords = {calculus, milner, pi, pi-calculus},
	Month = {June},
	Posted-At = {2008-01-08 16:12:29},
	Priority = {2},
	Publisher = {Cambridge University Press},
	Title = {Communicating and Mobile Systems: the Pi-Calculus},
	Url = {http://www.amazon.com/exec/obidos/redirect?tag=citeulike07-20&path=ASIN/0521658691},
	Year = {1999},
	Bdsk-Url-1 = {http://www.amazon.com/exec/obidos/redirect?tag=citeulike07-20&path=ASIN/0521658691}}

@article{modelchecking01,
	Abstract = {The aim of this paper is to illustrate by an example, the alternating
	bit protocol, the use of CESAR, an interactive system for aiding
	the design of distributed applications.},
	Author = {J. Queille and J. Sifakis},
	Citeulike-Article-Id = {2882655},
	Citeulike-Linkout-0 = {http://dx.doi.org/10.1007/3-540-11494-7_22},
	Citeulike-Linkout-1 = {http://www.springerlink.com/content/7x327643572334rw},
	Date-Added = {2010-08-03 14:46:55 +0200},
	Date-Modified = {2010-08-03 14:46:55 +0200},
	Doi = {10.1007/3-540-11494-7_22},
	Journal = {International Symposium on Programming},
	Keywords = {model\_checking, temporal\_logic},
	Pages = {337--351},
	Posted-At = {2009-01-22 23:02:58},
	Priority = {2},
	Title = {Specification and verification of concurrent systems in CESAR},
	Url = {http://dx.doi.org/10.1007/3-540-11494-7_22},
	Year = {1982},
	Bdsk-Url-1 = {http://dx.doi.org/10.1007/3-540-11494-7_22}}

@article{Lumpability1,
	Author = {P. Buchholz},
	Date-Added = {2010-08-03 14:46:54 +0200},
	Date-Modified = {2010-08-03 14:46:54 +0200},
	Journal = {Journal of applied probability, Applied Probability Trust},
	Pages = {59-75},
	Title = {Exact and Ordinary Lumpability in Finite Markov Chains},
	Volume = {31:11},
	Year = {1994}}

@article{HOG,
	Author = {Edda Klipp},
	Citeulike-Article-Id = {274184},
	Citeulike-Linkout-0 = {http://dx.doi.org/10.1038/nbt1114},
	Citeulike-Linkout-1 = {http://dx.doi.org/10.1038/nbt1114},
	Citeulike-Linkout-2 = {http://view.ncbi.nlm.nih.gov/pubmed/16025103},
	Citeulike-Linkout-3 = {http://www.hubmed.org/display.cgi?uids=16025103},
	Date-Added = {2010-08-03 14:46:54 +0200},
	Date-Modified = {2010-08-03 14:46:54 +0200},
	Doi = {10.1038/nbt1114},
	Issn = {1087-0156},
	Journal = {Nature Biotechnology},
	Keywords = {osmotic, pressure, yeast},
	Month = {July},
	Number = {8},
	Pages = {975--982},
	Posted-At = {2009-01-05 10:21:31},
	Priority = {2},
	Publisher = {Nature Publishing Group},
	Title = {Integrative model of the response of yeast to osmotic shock},
	Url = {http://dx.doi.org/10.1038/nbt1114},
	Volume = {23},
	Year = {2005},
	Bdsk-Url-1 = {http://dx.doi.org/10.1038/nbt1114}}

@article{HC3,
	Author = {H. Conzelmann and E.D. Gilles},
	Date-Added = {2010-08-03 14:46:53 +0200},
	Date-Modified = {2010-08-03 14:46:53 +0200},
	Journal = {Methods in Molecular Biology},
	Owner = {petrov},
	Pages = {559-578},
	Timestamp = {2009.07.03},
	Title = {Dynamic Pathway Modeling of Signal Transduction Networks: A Domain-Oriented Approach},
	Volume = {484},
	Year = {2008}}

@article{HC2,
	Abstract = {Abstract Background Receptors and scaffold proteins usually possess
	a high number of distinct binding domains inducing the formation
	of large multiprotein signaling complexes. Due to combinatorial reasons
	the number of distinguishable species grows exponentially with the
	number of binding domains and can easily reach several millions.
	Even by including only a limited number of components and binding
	domains the resulting models are very large and hardly manageable.
	A novel model reduction technique allows the significant reduction
	and modularization of these models. Results We introduce methods
	that extend and complete the already introduced approach. For instance,
	we provide techniques to handle the formation of multi-scaffold complexes
	as well as receptor dimerization. Furthermore, we discuss a new modeling
	approach that allows the direct generation of exactly reduced model
	structures. The developed methods are used to reduce a model of EGF
	and insulin receptor crosstalk comprising 5,182 ordinary differential
	equations (ODEs) to a model with 87 ODEs. Conclusion The methods,
	presented in this contribution, significantly enhance the available
	methods to exactly reduce models of combinatorial reaction networks.},
	Author = {H. Conzelmann and D. Fey and E.D. Gilles},
	Date-Added = {2010-08-03 14:46:52 +0200},
	Date-Modified = {2010-08-03 14:46:52 +0200},
	Institution = {BioMed Central [http://www.biomedcentral.com/oai/2.0/] (United Kingdom)},
	Journal = {BMC Systems Biology},
	Publisher = {BioMed Central Ltd.},
	Title = {Exact model reduction of combinatorial reaction networks},
	Url = {http://www.biomedcentral.com/1752-0509/2/78},
	Volume = {2},
	Year = {2008},
	Bdsk-Url-1 = {http://www.biomedcentral.com/1752-0509/2/78}}

@article{HC1,
	Author = {Holger Conzelmann and Julio Saez-Rodriguez and Thomas Sauter and Boris N. Kholodenko and Ernst Dieter Gilles},
	Bibsource = {DBLP, http://dblp.uni-trier.de},
	Date-Added = {2010-08-03 14:46:51 +0200},
	Date-Modified = {2010-08-03 14:46:51 +0200},
	Ee = {http://dx.doi.org/10.1186/1471-2105-7-34},
	Journal = {BMC Bioinformatics},
	Pages = {34},
	Title = {A domain-oriented approach to the reduction of combinatorial complexity in signal transduction networks},
	Volume = {7},
	Year = {2006}}

@article{Gillespie,
	Author = {D.T. Gillespie},
	Date-Added = {2010-08-03 14:46:49 +0200},
	Date-Modified = {2010-08-03 14:46:49 +0200},
	Journal = {Journal of Physical Chemistry},
	Owner = {petrov},
	Pages = {2340-2361},
	Timestamp = {2009.07.01},
	Title = {Exact stochastic simulation of coupled chemical reactions},
	Volume = {81},
	Year = {1977}}

@article{GibbsMetrics,
	Author = {A. Gibbs and F. Su},
	Date-Added = {2010-08-03 14:46:47 +0200},
	Date-Modified = {2010-08-03 14:46:47 +0200},
	Journal = {International Statistical Review (2002)},
	Number = {3},
	Pages = {419-435},
	Title = {On choosing and bounding probability metrics},
	Url = {citeseer.ist.psu.edu/article/gibbs00choosing.html},
	Volume = {70},
	Year = {2002},
	Bdsk-Url-1 = {citeseer.ist.psu.edu/article/gibbs00choosing.html}}

@article{Gamma,
	Address = {New York, NY, USA},
	Author = {Jean-Pierre Ban\^{a}tre and Daniel Le M\'{e}tayer},
	Date-Added = {2010-08-03 14:46:46 +0200},
	Date-Modified = {2010-08-03 14:46:46 +0200},
	Doi = {http://doi.acm.org/10.1145/151233.151242},
	Issn = {0001-0782},
	Journal = {Communications ACM},
	Number = {1},
	Pages = {98--111},
	Publisher = {ACM},
	Title = {Programming by multiset transformation},
	Volume = {36},
	Year = {1993},
	Bdsk-Url-1 = {http://doi.acm.org/10.1145/151233.151242}}

@article{FH07,
	Author = {J. Fisher and T.A. Henzinger},
	Citeulike-Article-Id = {1885378},
	Citeulike-Linkout-0 = {http://dx.doi.org/10.1038/nbt1356},
	Citeulike-Linkout-1 = {http://dx.doi.org/10.1038/nbt1356},
	Citeulike-Linkout-2 = {http://view.ncbi.nlm.nih.gov/pubmed/17989686},
	Citeulike-Linkout-3 = {http://www.hubmed.org/display.cgi?uids=17989686},
	Date-Added = {2010-08-03 14:46:41 +0200},
	Date-Modified = {2010-08-03 14:46:41 +0200},
	Doi = {10.1038/nbt1356},
	Journal = {Nature Biotechnology},
	Keywords = {model, motivation},
	Month = {November},
	Number = {11},
	Pages = {1239--1249},
	Posted-At = {2009-06-22 07:43:59},
	Priority = {2},
	Publisher = {Nature Publishing Group},
	Title = {Executable cell biology},
	Url = {http://dx.doi.org/10.1038/nbt1356},
	Volume = {25},
	Year = {2007},
	Bdsk-Url-1 = {http://dx.doi.org/10.1038/nbt1356}}

@article{DoyenHenzinger08,
	Author = {Doyen, L. and Henzinger, T.A. and Raskin, J.-F.},
	Date-Added = {2010-08-03 14:46:40 +0200},
	Date-Modified = {2010-08-03 14:46:40 +0200},
	Journal = {Inernational Journal of Foundations of Computer Science},
	Number = {3},
	Pages = {549-563},
	Publisher = {World Scientific},
	Title = {Equivalence of Labeled Markov Chains},
	Volume = {19},
	Year = {2008}}

@article{crosstalk01,
	Abstract = {Cells must respond specifically to different environmental stimuli
	in order to survive. The signal transduction pathways involved in
	sensing these stimuli often share the same or homologous proteins.
	Despite potential cross-wiring, cells show specificity of response.
	We show, through modeling, that the physiological response of such
	pathways exposed to simultaneous and temporally ordered inputs can
	demonstrate system-level mechanisms by which pathways achieve specificity.
	We apply these results to the hyperosmolar and pheromone mitogen-activated
	protein (MAP) kinase pathways in the yeast Saccharomyces cerevisiae.
	These two pathways specifically sense osmolar and pheromone signals,
	despite sharing a MAPKKK, Ste11, and having homologous MAPKs (Fus3
	and Hog1). We show that in a single cell, the pathways are bistable
	over a range of inputs, and the cell responds to only one stimulus
	even when exposed to both. Our results imply that these pathways
	achieve specificity by filtering out spurious cross-talk through
	mutual inhibition. The variability between cells allows for heterogeneity
	of the decisions.},
	Address = {[1] FAS Center for Systems Biology, Harvard University, Cambridge, Massachusetts 02138, USA. [2] Division of Engineering and Applied Sciences, Harvard University, Cambridge, Massachusetts 02138, USA.},
	Author = {M. McClean},
	Citeulike-Article-Id = {1097014},
	Citeulike-Linkout-0 = {http://dx.doi.org/10.1038/ng1957},
	Citeulike-Linkout-1 = {http://dx.doi.org/10.1038/ng1957},
	Citeulike-Linkout-2 = {http://view.ncbi.nlm.nih.gov/pubmed/17259986},
	Citeulike-Linkout-3 = {http://www.hubmed.org/display.cgi?uids=17259986},
	Date-Added = {2010-08-03 14:46:39 +0200},
	Date-Modified = {2010-08-03 14:46:39 +0200},
	Doi = {10.1038/ng1957},
	Issn = {1061-4036},
	Journal = {Nature Genetics},
	Keywords = {crosstalk, network, pathway, signalling, yeast},
	Month = {January},
	Posted-At = {2007-03-08 15:55:05},
	Priority = {2},
	Title = {Cross-talk and decision making in MAP kinase pathways.},
	Url = {http://dx.doi.org/10.1038/ng1957},
	Year = {2007},
	Bdsk-Url-1 = {http://dx.doi.org/10.1038/ng1957}}

@inproceedings{CousotAI,
	Address = {London, UK},
	Author = {Cousot, Patrick},
	Booktitle = {Informatics - 10 Years Back. 10 Years Ahead.},
	Date-Added = {2010-08-03 14:46:38 +0200},
	Date-Modified = {2010-08-03 14:46:38 +0200},
	Isbn = {3-540-41635-8},
	Pages = {138--156},
	Publisher = {Springer-Verlag},
	Title = {Abstract Interpretation Based Formal Methods and Future Challenges},
	Year = {2001}}

@article{conf/vmcai/DanosFFK08,
	Author = {Vincent Danos and J{\`E}r{\`U}me Feret and Walter Fontana and Jean Krivine},
	Booktitle = {VMCAI},
	Crossref = {conf/vmcai/2008},
	Date = {2008-03-03},
	Date-Added = {2010-08-03 14:46:38 +0200},
	Date-Modified = {2010-08-03 14:46:38 +0200},
	Editor = {Francesco Logozzo and Doron Peled and Lenore D. Zuck},
	Ee = {http://dx.doi.org/10.1007/978-3-540-78163-9_11},
	Interhash = {264e8b71ebd87631100f7a22557121ae},
	Intrahash = {8a95e43c613c318ffa50beb539fc5430},
	Isbn = {978-3-540-78162-2},
	Journal = {Lecture Notes in Computer Science},
	Pages = {83-97},
	Publisher = {Springer},
	Series = {Lecture Notes in Computer Science},
	Title = {Abstract Interpretation of Cellular Signalling Networks.},
	Url = {http://dblp.uni-trier.de/db/conf/vmcai/vmcai2008.html#DanosFFK08},
	Volume = {4905},
	Year = {2008},
	Bdsk-Url-1 = {http://dblp.uni-trier.de/db/conf/vmcai/vmcai2008.html#DanosFFK08}}

@book{BolchMC,
	Author = {Gunter Bolch and Stefan Greiner and Hermann Meer and Kishor S. Trivedi},
	Date-Added = {2010-08-03 14:46:37 +0200},
	Date-Modified = {2010-08-03 14:46:37 +0200},
	Editor = {Wiley-Interscience},
	Publisher = {Springer},
	Title = {Queing Networks and Markov Chains: Modeling and Performance with Computer Science Applications},
	Year = {2006}}

@inproceedings{BioLab,
	Address = {Berlin, Heidelberg},
	Author = {E.M. Clarke and J.R. Faeder and C.J. Langmead and L.A. Harris, and S.K.Jha and A.Legay},
	Booktitle = {CMSB '08: Proceedings of the 6th International Conference on Computational Methods in Systems Biology},
	Date-Added = {2010-08-03 14:46:36 +0200},
	Date-Modified = {2010-08-03 14:46:36 +0200},
	Doi = {http://dx.doi.org/10.1007/978-3-540-88562-7_18},
	Isbn = {978-3-540-88561-0},
	Location = {Rostock, Germany},
	Pages = {231--250},
	Publisher = {Springer-Verlag},
	Title = {Statistical Model Checking in BioLab: Applications to the Automated Analysis of T-Cell Receptor Signaling Pathway},
	Year = {2008},
	Bdsk-Url-1 = {http://dx.doi.org/10.1007/978-3-540-88562-7_18}}

@article{IJSI,
	Author = {J\'er\^ome Feret and Heinz Koeppl and Tatjana Petrov},
	Date-Added = {2010-08-03 14:45:31 +0200},
	Date-Modified = {2010-08-03 14:45:31 +0200},
	Journal = {Int.\,Jour.\,of Software and Informatics},
	Note = {to appear},
	Title = {Stochastic fragments: A framework for the exact reduction of the stochastic semantics of rule-based models}}

@article{borisov,
	Author = {N.M{.} Borisov and N.I{.} Markevich and B.N.Kholodenko and E.Dieter Gilles},
	Date-Added = {2010-08-03 14:45:30 +0200},
	Date-Modified = {2010-08-03 14:45:30 +0200},
	Journal = {Biophysical Journal},
	Publisher = {The Biophysical Society},
	Title = {Signaling through Receptors and Scaffolds: Independent Interactions Reduce Combinatorial Complexity},
	Volume = {89},
	Year = {2005}}

@inproceedings{aplas2007,
	Author = {Vincent Danos and J{\'e}r{\^o}me Feret and Walter Fontana and Jean Krivine},
	Bibsource = {DBLP, http://dblp.uni-trier.de},
	Booktitle = {APLAS$\,$2007},
	Crossref = {DBLP:conf/aplas/2007},
	Date-Added = {2010-08-03 14:45:27 +0200},
	Date-Modified = {2010-08-03 14:45:27 +0200},
	Ee = {http://dx.doi.org/10.1007/978-3-540-76637-7_10},
	Title = {Scalable Simulation of Cellular Signaling Networks}}

@book{cauchy,
	Address = {New York, NY},
	Author = {Ince, Edward Lindsay},
	Date-Added = {2010-08-03 14:45:24 +0200},
	Date-Modified = {2010-08-03 14:45:24 +0200},
	Publisher = {Dover Publications, Inc.},
	Title = {Ordinary Differential Equations},
	Year = 1956}

@inproceedings{progress03,
	Author = {A. Sokolova and Vink, E.P. de},
	Booktitle = {Proc. PROGRESS Workshop 2003},
	Date-Added = {2010-08-03 14:45:22 +0200},
	Date-Modified = {2010-08-03 14:45:22 +0200},
	Publisher = {STW, Utrecht},
	Title = {On Relational Properties of Lumpability},
	Year = 2003}

@phdthesis{Conzelmann:thesis,
	Author = {H.Conzelmann},
	Date-Added = {2010-08-03 14:45:21 +0200},
	Date-Modified = {2010-08-03 14:45:21 +0200},
	School = {Institut f\"ur Systemdynamik des Universit\"at Stuttgart},
	Title = {Mathematical Modeling of Cellular Signal Transduction Pathways --- A Domain-Oriented Approach to Reduce Combinatorial Complexity},
	Year = {2008}}

@article{conzelmann:08,
	Author = {Conzelmann, H. and Fey, D. and Gilles, E.D.},
	Date-Added = {2010-08-03 14:45:19 +0200},
	Date-Modified = {2010-08-03 14:45:19 +0200},
	Journal = {BMC Systems Biology},
	Title = {Exact model reduction of combinatorial reaction networks},
	Volume = 2,
	Year = 2008}

@article{buchholz:94,
	Author = {Buchholz, Peter},
	Date-Added = {2010-08-03 14:45:17 +0200},
	Date-Modified = {2010-08-03 14:45:17 +0200},
	Journal = {Journal of Applied Probability},
	Number = {1},
	Publisher = {Applied Probability Trust},
	Title = {Exact and Ordinary Lumpability in Finite {M}arkov Chains},
	Volume = {31},
	Year = {1994}}

@article{borisov:08,
	Author = {Borisov, N.M. and Chistopolsky, A.S. and Faeder, J.R. and Kholodenko, B.N.},
	Date-Added = {2010-08-03 14:45:17 +0200},
	Date-Modified = {2010-08-03 14:45:17 +0200},
	Journal = {IET Syst.Biol.},
	Title = {Domain-oriented reduction of rule-based network models},
	Volume = 2,
	Year = 2008}

@article{1347609,
	Address = {Essex, UK},
	Annote = {Here .},
	Author = {Buchholz, Peter},
	Date-Added = {2010-08-03 14:45:13 +0200},
	Date-Modified = {2010-08-03 14:55:51 +0200},
	Journal = {Theor.Comp.Science},
	Number = {1-3},
	Publisher = {Elsevier Science Publishers Ltd.},
	Title = {Bisimulation relations for weighted automata},
	Volume = {393},
	Year = {2008}}

@inproceedings{lics2010,
	Author = {Vincent Danos and J\'er\^ome Feret and Walter Fontana and Russell Harmer and Jean Krivine},
	Booktitle = {LICS$\,$2010},
	Date-Added = {2010-08-03 14:44:49 +0200},
	Date-Modified = {2010-08-03 14:44:49 +0200},
	Note = {to appear},
	Title = {Abstracting the differential semantics of rule-based models: exact and automated model reduction}}

@article{conzelmann,
	Author = {H.Conzelmann and J.Saez-Rodriguez and T.Sauter and B.N.Kholodenko and E.{D.} Gilles},
	Date-Added = {2010-08-03 14:44:42 +0200},
	Date-Modified = {2010-08-03 14:44:42 +0200},
	Journal = {BMC Bioinformatics},
	Title = {A domain-oriented approach to the reduction of combinatorial complexity in signal transduction networks},
	Volume = {7},
	Year = {2006}}

@article{pnas,
	Author = {Feret, J\'{e}r\^{o}me and Danos, Vincent and Krivine, Jean and Harmer, Russ and Fontana, Walter},
	Doi = {10.1073/pnas.0809908106},
	Journal = {Proceedings of the National Academy of Sciences},
	Keywords = {modeling, systems-biology},
	Month = {April},
	Number = {16},
	Pages = {6453--6458},
	Title = {Internal coarse-graining of molecular systems},
	Url = {http://dx.doi.org/10.1073/pnas.0809908106},
	Volume = {106},
	Year = {2009},
	Bdsk-Url-1 = {http://dx.doi.org/10.1073/pnas.0809908106}}

@inproceedings{aplas,
	Author = {Vincent Danos and J{\'e}r{\^o}me Feret and Walter Fontana and Jean Krivine},
	Bibsource = {DBLP, http://dblp.uni-trier.de},
	Booktitle = {APLAS},
	Crossref = {DBLP:conf/aplas/2007},
	Ee = {http://dx.doi.org/10.1007/978-3-540-76637-7_10},
	Pages = {139-157},
	Title = {Scalable Simulation of Cellular Signaling Networks},
	Year = {2007}}

@proceedings{DBLP:conf/aplas/2007,
	Bibsource = {DBLP, http://dblp.uni-trier.de},
	Booktitle = {APLAS},
	Editor = {Zhong Shao},
	Isbn = {978-3-540-76636-0},
	Publisher = {Springer},
	Series = {Lecture Notes in Computer Science},
	Title = {Programming Languages and Systems, 5th Asian Symposium, APLAS 2007, Singapore, November 29-December 1, 2007, Proceedings},
	Volume = {4807},
	Year = {2007}}

@article{Buchholz,
	Author = {Peter Buchholz},
	Journal = {Journal of Applied Probability},
	Pages = {59--75},
	Title = {Exact and ordinary lumpability of finite {M}arkov chains},
	Volume = {31},
	Year = {1994}}

@article{Kappa,
	Author = {Vincent Danos and Cosimo Laneve},
	Journal = {Theoretical Computer Science},
	Pages = {69--110},
	Title = {Core Formal Molecular Biology},
	Volume = {325},
	Year = {2003}}

@article{bli:06,
	Author = {Michael L. Blinov and James R. Faeder and Byron Goldstein and William S. Hlavacek},
	Journal = {BioSystems},
	Month = Jan,
	Pages = {136--151},
	Title = {A network model of early events in epidermal growth factor receptor signaling that accounts for combinatorial complexity},
	Volume = 83,
	Year = 2006}

@inproceedings{VMCAI08,
	Author = {Vincent Danos and J{\'e}r{\^o}me Feret and Walter Fontana and Jean Krivine},
	Booktitle = {Proceedings of the 9th International Conference on Verification, Model Checking and Abstract Interpretation (VMCAI'08)},
	Pages = {42-58},
	Title = {Abstract Interpretation of Reachable Complexes in Biological Signalling Networks},
	Volume = {4905},
	Year = {2008}}

@inproceedings{fmsb:2008,
	Author = {Vincent Danos and J{\'er\^o}me Feret and Walter Fontana and Russel Harmer and Jean Krivine},
	Booktitle = {Proceedings of Formal Methods in Systems Biology (FMSB'08)},
	Series = {LNBI},
	Title = {Rule-based modelling, symmetries, refinements},
	Year = {2008}}

@incollection{ecsb:2009,
	Author = {Elaine Murphy and Vincent Danos and Jerome Feret and Russell Harmer and Jean Krivine},
	Booktitle = {Elements of Computational Systems Biology},
	Editor = {Huma Lodhi and Stephen Muggleton},
	Publisher = {Wiley Book Series on Bioinformatics},
	Title = {Rule Based Modelling and Model Refinement},
	Year = {2009}}

@book{walshct_2006,
	Author = {Walsh, Christopher T.},
	Publisher = {Roberts and Co. Publisher},
	Title = {Posttranslation Modification of Proteins: Expanding Nature's Inventory},
	Year = {2006}}

@book{lattices,
	Author = {Davey, B.A.},
	Publisher = {University of Oxford},
	Title = {Introduction to Lattices and Order},
	Year = {2002}}

@inproceedings{Regev1,
	Address = {Singapore},
	Author = {Aviv Regev and William Silverman and Ehud Shapiro},
	Booktitle = {Pacific Symposium on Biocomputing},
	Date-Added = {2007-01-30 10:07:22 -0500},
	Date-Modified = {2007-07-27 02:55:23 -0400},
	Editor = {R. B. Altman and A. K. Dunker and L. Hunter and T. E. Klein},
	Keywords = {logic, pi-calculus, signaling, semi-quantitative, implementation, simulation, BioPSI, calculus, executable, mutation, formal verification},
	Pages = {459--470},
	Publisher = {World Scientific Press},
	Title = {Representation and Simulation of Biochemical Processes Using the {$\pi$}-Calculus Process Algebra},
	Volume = {6},
	Year = {2001}}

@book{Mil99,
	Address = {Cambridge},
	Author = {Robin Milner},
	Date-Added = {2007-01-30 10:07:30 -0500},
	Date-Modified = {2007-04-03 14:42:21 +0100},
	Publisher = {Cambridge University Press},
	Title = {Communicating and mobile systems: the $\pi$-calculus},
	Year = 1999}

@inproceedings{Lincoln,
	Author = {Steven Eker and Merrill Knapp and Keith Laderoute and Patrick Lincoln and Jos{\'e} Meseguer and Kemal Sonmez},
	Booktitle = {Proceedings of the Pacific Symposium on Biocomputing},
	Date-Added = {2007-01-30 10:07:22 -0500},
	Date-Modified = {2007-07-27 02:55:53 -0400},
	Month = {January},
	Pages = {400-412},
	Title = {Pathway Logic: Symbolic Analysis of Biological Signaling},
	Year = {2002}}

@article{regev2004bab,
	Author = {Regev, Aviv and Panina, Ekaterina M. and Silverman, William and Cardelli, Luca and Shapiro, Ehud},
	Date-Added = {2007-06-23 09:59:39 -0400},
	Date-Modified = {2007-07-15 16:23:13 -0400},
	Journal = {Theoretical Computer Science},
	Number = {1},
	Pages = {141--167},
	Title = {{BioAmbients: an abstraction for biological compartments}},
	Volume = {325},
	Year = {2004}}

@inproceedings{branecalc,
	Author = {Luca Cardelli},
	Booktitle = {Proceedings of BIO-CONCUR'03, Marseille, France},
	Date-Added = {2007-01-30 10:07:30 -0500},
	Date-Modified = {2007-06-23 09:54:21 -0400},
	Issue = {3},
	Publisher = {Elsevier},
	Series = {Electronic Notes in Theoretical Computer Science},
	Title = {Brane Calculi},
	Volume = {180},
	Year = {2003}}

@inproceedings{dk:fmbccs,
	Author = {Vincent Danos and Jean Krivine},
	Booktitle = {Proceedings of BIO-CONCUR'03, Marseille, France},
	Date-Modified = {2007-07-20 13:57:10 -0400},
	Issue = {3},
	Pages = {31--49},
	Publisher = {Elsevier},
	Series = {Electronic Notes in Theoretical Computer Science},
	Title = {Formal Molecular Biology done in {CCS}},
	Volume = {180},
	Year = {2003}}

@incollection{shapirobe_2001,
	Author = {Shapiro, Bruce E. and Levchenko, Andre and Mjolsness, Eric},
	Booktitle = {Foundations of Systems Biology},
	Chapter = {1},
	Editor = {Kitano, H.},
	Publisher = {MIT Press},
	Title = {Automatic model generation for signal transduction with application to {MAP} kinase pathways},
	Year = {2001}}

@article{lokl_2005,
	Author = {Lok, Larry and Brent, Roger},
	Journal = {Nat Biotechn},
	Pages = {131-136},
	Title = {Automatic generation of cellular reaction networks with Moleculizer 1.0},
	Volume = {1},
	Year = {2005}}

@phdthesis{thomsontm_2008_2,
	Address = {Cambridge MA, USA},
	Author = {Thomson, Ty M.},
	School = {Massachusetts Institute of Technology (MIT)},
	Title = {Models and analysis of yeast mating response : tools for model building, from documentation to time-dependent stimulation},
	Year = {2008}}

@article{hlavacek2006rms,
	Author = {Hlavacek, William S. and Faeder, James R. and Blinov, Michael L. and Posner, Richard G. and Hucka, Michael and Fontana, Walter},
	Date-Added = {2007-01-30 10:07:30 -0500},
	Date-Modified = {2007-04-03 14:42:21 +0100},
	Journal = {Science's STKE},
	Number = {344},
	Title = {{Rules for Modeling Signal-Transduction Systems}},
	Volume = {2006},
	Year = {2006}}

@article{conzelmannh_2008_1,
	Author = {Conzelmann, Holger and Fey, Dirk and Gilles, Ernst D.},
	Journal = {BMC Syst Biol},
	Number = {78},
	Pages = {342--351},
	Title = {Exact model reduction of combinatorial reaction},
	Volume = {2},
	Year = {2008}}

@article{Gillespie1977,
	Author = {Daniel T. Gillespie},
	Journal = {J Phys Chem},
	Number = {25},
	Pages = {2340-2361},
	Title = {Exact Stochastic Simulation of Coupled Chemical Reactions},
	Volume = {81},
	Year = {1977}}

@article{hlavacekws_2003,
	Author = {Hlavacek, William S. and Faeder, James R. and Blinov, Michael L. and Perelson, Alan S. and Goldstein, Byron},
	Journal = {Biotechnol. Bio-eng.},
	Pages = {783--794},
	Title = {The complexity of complexes in signal transduction},
	Volume = {84},
	Year = {2005}}

@book{wilkinsondj_2006,
	Author = {Wilkinson, Darren J.},
	Publisher = {Chapman \& Hall},
	Title = {Stochastic Modelling for Systems Biology},
	Year = {2006}}

@article{blinov2004,
	Author = {Blinov, Michael L. and Faeder, James R. and Hlavacek, William S.},
	Date-Added = {2007-01-30 10:07:30 -0500},
	Date-Modified = {2007-04-03 14:42:21 +0100},
	Journal = {Bioinformatics},
	Pages = {3289-3292},
	Title = {{BioNetGen: software for rule-based modeling of signal transduction based on the interactions of molecular domains}},
	Volume = {20},
	Year = {2004}}

@inproceedings{concur2007,
	Address = {Lisbon, Portugal},
	Author = {Vincent Danos and J{\'e}r{\^o}me Feret and Walter Fontana and Russ Harmer and Jean Krivine},
	Booktitle = {Proceedings of the Eighteenth International Conference on Concurrency Theory, CONCUR$\,$'2007, Lisbon, Portugal},
	Month = {3--8 September},
	Pages = {17--41},
	Publisher = {Springer, Berlin, Germany},
	Series = {Lecture Notes in Computer Science},
	Title = {Rule-Based Modelling of Cellular Signalling, invited paper},
	Volume = {4703},
	Year = {2007}}

@article{gb:97,
	Address = {New York, NY, USA},
	Author = {Cortesi, Agostino and Fil\'{e}, Gilberto and Ranzato, Francesco and Giacobazzi, Roberto and Palamidessi, Catuscia},
	Doi = {http://doi.acm.org/10.1145/239912.239914},
	Issn = {0164-0925},
	Journal = {ACM Trans. Program. Lang. Syst.},
	Number = {1},
	Pages = {7--47},
	Publisher = {ACM},
	Title = {Complementation in abstract interpretation},
	Volume = {19},
	Year = {1997},
	Bdsk-Url-1 = {http://doi.acm.org/10.1145/239912.239914}}

@phdthesis{c:thesis,
	Address = {Gre\-no\-ble, Fran\-ce},
	Author = {Cousot, Patrick},
	Month = {21 March},
	School = {Uni\-ver\-si\-t{\'e} Jo\-seph Fou\-r\-ier},
	Title = {M{\'e}\-tho\-des it{\'e}\-ra\-ti\-ves de cons\-truc\-tion et d'ap\-pro\-xi\-ma\-tion de points fi\-xes d'op{\'e}\-ra\-teurs mo\-no\-to\-nes sur un treil\-lis, ana\-ly\-se s{\'e}\-man\-ti\-que de pro\-gram\-mes (in {F}rench)},
	Type = {Th{\`e}\-se d'{{\'E}}tat {\`e}s sci\-en\-ces ma\-th{\'e}\-ma\-ti\-ques},
	Year = 1978}

@article{cc:92,
	Author = {Cousot, Patrick and Cousot, Radhia},
	Journal = {Journal of Logic and Computation},
	Number = 4,
	Pages = {511--547},
	Publisher = {Oxford University Press, Oxford, UK},
	Title = {Abstract Interpretation Frameworks},
	Volume = 2,
	Year = 1992}

@inproceedings{cc:77,
	Author = {Patrick Cousot and Radhia Cousot},
	Bibsource = {DBLP, http://dblp.uni-trier.de},
	Booktitle = {Conference Record of the Fourth Annual ACM SIGPLAN-SIGACT Symposium on Principles of Programming Languages},
	Pages = {238-252},
	Title = {Abstract Interpretation: A Unified Lattice Model for Static Analysis of Programs by Construction or Approximation of Fixpoints},
	Year = {1977}}

@inproceedings{cc:79,
	Address = {San Antonio, Texas},
	Author = {Cousot, Patrick and Cousot, Radhia},
	Booktitle = {Conference Record of the Sixth Annual ACM SIGPLAN-SIGACT Symposium on Principles of Programming Languages},
	Pages = {269--282},
	Publisher = {ACM Press, New York, NY},
	Title = {Systematic design of program analysis frameworks},
	Year = 1979}

@inproceedings{koepplh_2009_4,
	Address = {Aarhus, Denmark},
	Author = {Koeppl, Heinz and Schumacher, Linus and Danos, Vincent},
	Booktitle = {Proceedings of the sixth International Workshop on Computational Systems Biology (WCSB)},
	Month = {June 10-12},
	Pages = {95--98},
	Publisher = {TICSP},
	Title = {A statistical analysis of receptor clustering using random graphs},
	Volume = {48},
	Year = {2009}}

@techreport{Doyen09:probWA,
	Affiliation = {EPFL},
	Author = {Chatterjee, Krishnendu and Doyen, Laurent and Henzinger, Thomas A.},
	Details = {http://infoscience.epfl.ch/record/133665},
	Documenturl = {http://infoscience.epfl.ch/getfile.py?recid=133665&mode=best},
	Keywords = {Weighted automata; Probabilistic automata; Quantiative languages},
	Oai-Id = {oai:infoscience.epfl.ch:133665},
	Oai-Set = {report; fulltext-public; fulltext},
	Title = {Probabilistic {W}eighted {A}utomata},
	Unit = {MTC},
	Year = {2009}}

@misc{Hermanns99:weakbisimulation,
	Author = {Christel Baier and Holger Hermanns},
	Title = {Weak Bisimulation for Fully Probabilistic Processes},
	Year = {1999}}

@book{KS60:lump,
	Author = {Kemeny, John and Snell, James L.},
	Publisher = {Van Nostrand},
	Title = {Finite {M}arkov Chains},
	Year = {1960}}

@inproceedings{LS89:ProbBis,
	Address = {New York, NY, USA},
	Author = {Larsen, Kim G. and Skou, Arne},
	Booktitle = {POPL '89: Proceedings of the 16th ACM SIGPLAN-SIGACT symposium on Principles of programming languages},
	Doi = {http://doi.acm.org/10.1145/75277.75307},
	Isbn = {0-89791-294-2},
	Location = {Austin, Texas, United States},
	Pages = {344--352},
	Publisher = {ACM},
	Title = {Bisimulation through probabilistic testing (preliminary report)},
	Year = {1989},
	Bdsk-Url-1 = {http://doi.acm.org/10.1145/75277.75307}}

@book{book:bolch-queueingnetworks06,
	Author = {Bolch, Gunter and Greiner, Stefan and de Meer, Hermann and Trivedi, Kishor S.},
	Edition = {2nd Edition},
	Howpublished = {Hardcover},
	Isbn = {0471565253},
	Keywords = {analysis, bolch, networks, performance, queueing, throughput},
	Month = {May},
	Posted-At = {2009-07-03 20:02:39},
	Priority = {2},
	Publisher = {WileyBlackwell},
	Title = {Queueing Networks and {M}arkov Chains: Modeling and Performance Evaluation with Computer Science Applications},
	Url = {http://www.amazon.com/exec/obidos/redirect?tag=citeulike07-20&path=ASIN/0471565253},
	Year = {2006},
	Bdsk-Url-1 = {http://www.amazon.com/exec/obidos/redirect?tag=citeulike07-20&path=ASIN/0471565253}}

@article{PP:BisimulLMP02,
	Address = {Duluth, MN, USA},
	Author = {Desharnais, Jos\'{e}e and Edalat, Abbas and Panangaden, Prakash},
	Doi = {http://dx.doi.org/10.1006/inco.2001.2962},
	Issn = {0890-5401},
	Journal = {Inf. Comput.},
	Number = {2},
	Pages = {163--193},
	Publisher = {Academic Press, Inc.},
	Title = {Bisimulation for labelled {M}arkov processes},
	Volume = {179},
	Year = {2002},
	Bdsk-Url-1 = {http://dx.doi.org/10.1006/inco.2001.2962}}

@article{Doyen:EMC08,
	Author = {Laurent Doyen and Thomas A. Henzinger and Jean-Fran\c{c}ois Raskin},
	Bibsource = {DBLP, http://dblp.uni-trier.de},
	Ee = {http://dx.doi.org/10.1142/S0129054108005814},
	Journal = {Int. J. Found. Comput. Sci.},
	Number = {3},
	Pages = {549-563},
	Title = {Equivalence of Labeled {M}arkov Chains},
	Volume = {19},
	Year = {2008}}

@inproceedings{SOS,
	Address = {London, UK},
	Author = {Bodei, Chiara and Degano, Pierpaolo and Priami, Corrado},
	Booktitle = {SAS '98: Proceedings of the 5th International Symposium on Static Analysis},
	Isbn = {3-540-65014-8},
	Pages = {168--183},
	Publisher = {Springer-Verlag},
	Title = {Constructing Specific SOS Semantics for Concurrency via Abstract Interpretation},
	Year = {1998}}

@article{mcquarrieda_1967_1,
	Author = {McQuarrie, Donald A.},
	Journal = {Journal of Applied Probability},
	Number = {3},
	Pages = {413-478},
	Title = {Stochastic approach to chemical kinetics},
	Volume = {4},
	Year = {1967}}

@inproceedings{Monniaux_SAS00,
	Author = {David Monniaux},
	Booktitle = {Proceeding of the Seventh International Static Analysis Symposium (SAS'00)},
	Category = {intc},
	Number = 1824,
	Pages = {322--339},
	Publisher = {Springer Verlag},
	Series = {LNCS},
	Title = {Abstract Interpretation of Probabilistic Semantics},
	Year = 2000}

@inproceedings{Monniaux_POPL01,
	Author = {David Monniaux},
	Booktitle = {Proceedings of the 28th Symposium on Principles of Programming Languages (POPL'01)},
	Category = {intc},
	Organization = {ACM},
	Pages = {93--101},
	Title = {An Abstract {M}onte-{C}arlo Method for the Analysis of Probabilistic Programs (extended abstract)},
	Year = 2001}

@article{LeviENTCS09,
	Author = {Coletta, Alessio and Gori, Roberta and Levi, Francesca},
	Journal = {ENTCS},
	Number = {1},
	Pages = {165--182},
	Publisher = {Elsevier Science Publishers B. V.},
	Title = {Approximating Probabilistic Behaviors of Biological Systems Using Abstract Interpretation},
	Volume = {229},
	Year = {2009}}

@inproceedings{wiklicky,
	Author = {{Di Pierro},, Alessandra and Wiklicky,, Herbert},
	Booktitle = {Proceedings of the Second Joint International Workshop on Process Algebra and Probabilistic Methods, Performance Modeling and Verification (PAPM-PROBMIV'02)},
	Pages = {211--212},
	Publisher = {Springer-Verlag},
	Title = {Probabilistic Abstract Interpretation and Statistical Testing},
	Year = {2002}}

@book{rachevst_1991_1,
	Address = {New York},
	Author = {Rachev, Svetlozar T.},
	Publisher = {Wiley},
	Series = {Probability and Mathematical Statistics},
	Title = {Probability metrics and the stability of stochastic models},
	Year = {1991}}

@article{desharnaisj_2004_1,
	Author = {Desharnais, Jos\'{e}e and Gupta, Vineet and Jagadeesan, Radha and Panangaden, Prakash},
	Journal = {Theoretical computer science},
	Number = {3},
	Pages = {323--354},
	Title = {Metrics for labelled {M}arkov processes},
	Volume = {318},
	Year = {2004}}

@inproceedings{thorsleyd_2008_1,
	Author = {Thorsley, David and Klavins, Eric},
	Booktitle = {Proceedings of the 2008 American Control Conference},
	Month = {June 11--13},
	Pages = {1374--1381},
	Title = {Model Reduction of Stochastic Processes Using {Wasserstein} Pseudometrics},
	Year = {2008}}

@article{pahlej_2009_1,
	Author = {Pahle, J{\"u}rgen},
	Journal = {Brief Bioinform},
	Number = {1},
	Pages = {53--64},
	Title = {Biochemical simulations: stochastic, approximate stochastic and hybrid approaches},
	Volume = {10},
	Year = {2009}}

@article{blinov:sim,
	Author = {Joshua Colvin and Michael I. Monine and James R. Faeder and William S. Hlavacek and Daniel D. Von Hoff and Richard G. Posner},
	Bibsource = {DBLP, http://dblp.uni-trier.de},
	Ee = {http://dx.doi.org/10.1093/bioinformatics/btp066},
	Journal = {Bioinformatics},
	Number = {7},
	Pages = {910-917},
	Title = {Simulation of large-scale rule-based models},
	Volume = {25},
	Year = {2009}}

@article{schoeberl,
	Author = {Schoeberl, Birgit and Eichler-Jonsson, Claudia and Gilles, Ernst D. and M\"{u}ller, Gertraud},
	Journal = {Nat Biotechnol},
	Month = {April},
	Number = {4},
	Pages = {370--375},
	Title = {Computational modeling of the dynamics of the MAP kinase cascade activated by surface and internalized EGF receptors.},
	Volume = {20},
	Year = {2002}}



@article{fb,
	Author = {Brightman, Frances A. and Fell, David A.},
	Journal = {FEBS Letters},
	Month = {October},
	Number = {3},
	Pages = {169--174},
	Title = {Differential feedback regulation of the MAPK cascade underlies the quantitative differences in EGF and NGF signalling in PC12 cells},
	Volume = {482},
	Year = {2000}}
	

@inproceedings{Ptrv2011,
  author = "Petrov, Tatjana and Koeppl, Heinz and Ganguly, Arnab",
  title = "{M}olecular {S}ignaling: {M}odel {D}ecomposition and {S}tochastic {F}ragments",
  year = 2011,
  publisher = "Second International Workshop on Static Analysis and Systems Biology",
}


@article{TCS-MeCBIC2012,
   author =    {J\'er\^ome Feret and Thomas Henzinger and  Heinz Koeppl and Tatjana Petrov},
   title =     {Lumpability Abstractions of Rule-based Systems},
   editor =    {G.~Ciobanu, M.~Koutny},
   journal =   {Theoretical Computer Science}, 
   year =      {2012},
}

@book{ref:Kei87,
    author = {Keizer, Joel},
    edition = {1},
    howpublished = {Hardcover},
    isbn = {0387965017},
    keywords = {chemical\_physics, noise, non-equilibrium, physics, statistical\_physics, textbook, thermodynamics},
    month = jul,
    priority = {2},
    publisher = {Springer},
    title = {{Statistical Thermodynamics of Nonequilibrium Processes}},
    year = {1987}
}

@article{ref:Gup95,
    address = {Centre for Cellular and Molecular Biology, Hyderabad-7, AP, India},
    author = {Guptasarma, P.},
    journal = {BioEssays : news and reviews in molecular, cellular and developmental biology},
    keywords = {bacteria, copy\_number, e\_coli, stochastic, transcription},
    month = nov,
    number = {11},
    pages = {987--997},
    pmid = {8526893},
    priority = {2},
    title = {{Does replication-induced transcription regulate synthesis of the myriad low copy number proteins of Escherichia coli?}},
    url = {http://dx.doi.org/10.1002/bies.950171112},
    volume = {17},
    year = {1995}
}

@article{ref:Yuetal06,
 title={Probing gene expression in live cells, one protein molecule at a time.}, volume={311}, url={http://www.ncbi.nlm.nih.gov/pubmed/16543458}, number={5767}, journal={Science}, publisher={AAAS}, author={Yu, J and Xiao, J and Ren, X and Lao, K and Xie, X S}, year={2006}, pages={1600--3}}
 
@article{ref:Friedman10,
author = {Nir Friedman and Long Cai and X. Sunney Xie},
title = {Stochasticity in Gene Expression as Observed by Single-molecule Experiments in Live Cells},
journal = {Israel Journal of Chemistry},
volume = {49},
year = {2010},
pages = {333--342},
doi = {10.1560/IJC.49.3-4.333},
masid = {24603057}
}


@book{ref:wilkinson_2006,
	Author 		= "D. J. Wilkinson",
	Title 		= "Stochastic Modelling for Systems Biology",
	Publisher 	= "Chapman \& Hall",
	Year 		= "2006",
}


@article{ref:Gillespie2007,
    author = {D. T. Gillespie},
    journal = {Annu Rev Phys Chem},
    number = {1},
    pages = {35--55},
    title = {Stochastic simulation of chemical kinetics},
    volume = {58},
    year = {2007},
}
	
@INCOLLECTION{ref:AndKur-11,
   AUTHOR       = {D. F. Anderson and T. G. Kurtz},
   BOOKTITLE    = {Design and Analysis of Biomolecular Circuits},
   PUBLISHER    = {Springer-Verlag},
   TITLE        = {Continuous time Markov chain models for chemical reaction networks},
   YEAR         = {2011},
   EDITOR       = {H. Koeppl and G. Setti and di Bernardo, M. and 
      D. Densmore},
      }
	
	
	
	

@comment{BibDesk URL Groups{
<?xml version="1.0" encoding="UTF-8"?>
<!DOCTYPE plist PUBLIC "-//Apple//DTD PLIST 1.0//EN" "http://www.apple.com/DTDs/PropertyList-1.0.dtd">
<plist version="1.0">
<array>
	<dict>
		<key>URL</key>
		<string>file://localhost/Users/petrov/Desktop/mfpsXXVI.bib</string>
		<key>group name</key>
		<string>mfpsXXVI.bib</string>
	</dict>
	<dict>
		<key>URL</key>
		<string>file://localhost/Users/petrov/Desktop/ref-1.bib</string>
		<key>group name</key>
		<string>ref-1.bib</string>
	</dict>
	<dict>
		<key>URL</key>
		<string>file://localhost/Users/petrov/Desktop/ref.bib</string>
		<key>group name</key>
		<string>ref.bib</string>
	</dict>
	<dict>
		<key>URL</key>
		<string>file://localhost/Users/petrov/Desktop/ref2.bib</string>
		<key>group name</key>
		<string>ref2.bib</string>
	</dict>
</array>
</plist>
}}




==> tex/approx_detailed.tex <==
%We focus on three interaction patterns where the reduction can be applied. These are: enzymatic reduction, dimerization reduction and operator site reduction.
%We consider several reduction... based on ...
%Our approach for obtaining approximate model consists in eliminating those species whose relative effect to the observable can be estimated by assuming that certain fast reactions are in equilibrium.
%The technique of separating the time scales of subsets of the reaction networks has gained considerable attention

In this section, we present the mathematical analysis underlying the approximation algorithms presented in \secref{algorithms}.
The basic idea is best illustrated over the elementary enzymatic transformation from a substrate $\subs$ to a product $\product$, through the intermediate complex $E:S$:
\begin{align}
\label{eq:mmreac}
\enz+\subs\rates{k_1}{k_2} \enz:\subs \rA{{k_3}} \enz+\product,
\end{align}
which our algorithm will convert to the well-known Michaelis-Menten form
\begin{align}	
\label{eq:mm}
\subs\rA{\frac{k_3 \enz_T K}{1+K\conc{S}}} \product,
\end{align}
%Whenever the complex formation is very fast comparing to the velocity of producing $\product$, 
%%The {Michaelis-Menten approximation} in this case refers to assuming
%one may approximate well the amount of product as only a function of substrate, by 
%assuming that the complex is in equilibrium.
%%of the substrate concentration and eliminating the intermediate reaction step. 
where $\enz_T=\conc{E}(t)+\conc{E:S}(t)$ denotes the total concentration of the enzyme, 
%$[\cdot]$ the concentration of the respective species, 
and $K=\frac{k_1}{k_2+{k_3}}$.  

The above approximation is generally considered to be sufficiently good, whenever the rate of complex formation is much faster than the complex dissociation (i.e. $k_1\gg k_2+k_3$), that is also known as the \emph{equilibrium approximation}.  
Even if the equilibrium condition is not satisfied, it can be compensated in a situation where the total number of substrates significantly outnumbers the enzyme concentration - ${\conc{S}(0)+K}\gg {\enz_T}$, known as the \emph{quasi-steady-state assumption}.

%\paragraph{Generalized enzymatic approximation - operator site reduction}
%This approximation is valid whenever the reaction of binding and unbinding between the substrate and the enzyme happens at a significantly faster time-scale than the conversion of the complex to the product. 
%The situation arises either when the rate of conversion to the substrate is much larger than the rate of the conversion to the product ($k_1^-\gg\hat{k_1}$), or when the enzyme co

Whenever one of the above assumptions holds, the quantity of the intermediate complex can be assumed to be rapidly reaching equilibrium, that is, $\deriv \conc{E:T}(t) =0$.
Then, it is straightforward to derive the rate of direct conversion from substrate to product:
\begin{align*}
\deriv\conc{\product} = \frac{k_3\enz_TK}{1+K\conc{S}}\conc{S},
\end{align*}
which exactly corresponds to the equation for the rule \eqref{eq:mm}.


The informal terminology of being `significantly faster', motivated the rigorous study of the limitations of the approximations based on separating time scales. 
%
While the enzymatic (Michaelis-Menten) approximation has been first introduced and subsequently studied in the context of deterministic models (e.g. \cite{murray2002mathematical}, Ch.6), it was more recently that the time-scale separation was investigated in the stochastic context \cite{rao2003stochastic}, \cite{haseltine2002approximate}, \cite{crudu2009hybrid}, \cite{hepp2014adaptive}, \cite{sanft2011legitimacy}, \cite{gillespie2009subtle}.
%, the authors study the limitations and caveats of using the time-scale separation in the stochastic setting. 
%
Notably, the following result from \cite{darden1979pseudo} (also shown as a special case of the framework in  \cite{kang2013separation}), shows that  
%over the kinetic parameters, total enzyme concentration and the cell volume, 
 the original model and the approximate model converge to the same process. 

It is worth noticing that this does not provide the means of computing the approximation error, or an algorithm which suggests which difference in time-scales is good enough for an approximation to perform well.
Rather, this result shows 
%t
%hat in the theoretical limit when the kinetic rates and species concentrations satisfy assumed relations, the approximate model is indeed a limit of the original one.
% provides mathematical rigour to the intuitive understanding that the approximation is good if the complex formation is rapid, the amount of substrate and the volume have the same order of magnitude, the total volume is large, and the amount of enzyme is not negligible with respect to the total volume.
%that the magnitude of total substrate count is larger than the one of the enzyme.
%the approximation gets better when the total enzyme.
% and \cite{myers2011engineering}.
%\thmref{thm:kang} shows 
that the enzymatic approximation is justified in the limit %when $\volume\ra\infty$ and 
when the assumptions about the reaction rates and species' abundance are met. 
%
In other words, in the theoretical limits of these assumptions, the original and reduced model are equivalent processes. % when appropriately scaled.
%



%\subsection{Approximation guarantees}
\newtheorem{theorem}{Theorem} 
\begin{theorem} (Darden \cite{darden1979pseudo}, Kang \cite{kang2013separation}). \rm
Consider the equation \eqref{eq:mmreac}, 
and denote by $X_{\subs}(t)$, $X_{\enz}(t)$, $X_{\enz:\subs}(t)$ and $X_{\product}(t)$ the 
copy numbers of the respective species due to the random-time change model \eqref{eq:rtc}.
Denote by $\enz_T = X_{\enz:\subs}(t)+X_{\enz}(t)$ and
$V_{\enz}(t) = \int_0^t \volume^{-1}X_{\enz}(s)\der s$
 and assume that $\volume = {\cal O}(X_{\subs})$. 
Assume that
$k_1\ra\gamma_1$,
$k_2/\volume \ra\gamma_2$,
$k_3/\volume \ra \gamma_3$,
$\volume\to\infty$, and
$\frac{X_{\subs}(0)}{\volume}\ra x_{\subs}(0)$.
Then $(\frac{X_{\subs}(t)}{\volume}, \Vel_{\enz}(t))$ converges to $(\conc{\subs}(t), \vel_{\enz}(t))$ and 
\[\deriv\vel_{\enz}(s) = \frac{\enz_T}{1+\hat{K}\conc{\enz}(s)}
\hbox{ \;\;\; and \;\;\;} 
\deriv\conc{\subs} = - \frac{\enz_T{\gamma_3} \hat{K}\conc{\subs}(t)}{1+\hat{K}\conc{\subs}(t)},
\]
where $\hat{K} = \frac{\gamma_1}{\gamma_2+{\gamma_3}}$.
\label{thm:kang}
\end{theorem}


The assumptions listed in the theorem capture the informal notion that:
(i) $X_{\subs}$ and $X_{\product}$ are scaled to concentrations, while $X_{\enz}$ and $X_{\enz:\subs}$ remain in copy numbers;
(ii) the reaction rate $k_1$ is larger than $k_2$ and that $k_3$ for an order of $\volume$. 

Before proceeding to the proof, we restate why the \thmref{thm:lang} justifies the reduction from \eqref{eq:mmreac} to \eqref{eq:mm}.
%
Notice that 
\[
\hat{K}\conc{\subs}(t) = \frac{\gamma_1}{\gamma_2+\gamma_3}\conc{\subs}(t)  = \frac{k_1}{\volume(k_2+k_3)}\conc{\subs}(t)  = K\frac{\conc{\subs}(t)}{\volume}.
\]

According to \eqref{eq:mm}, the random time change for the product is given by
\[
\hat{X}_{\product}(t) = \hat{X}_{\product}(0)+\int_0^t \frac{k_3\enz_{T} K}{1+K\hat{X}_{\subs}}\hat{X}_{\subs} \der s,
\]
while, according to \eqref{eq:mmreac}, the random time change for the product is given by
\[
{X}_{\product}(t) = {X}_{\product}(0)+\int_0^t k_3 {X}_{\enz:\subs}(s) \der s,
\]
where $X_{\enz:\subs}(t) = \enz_T-X_{\enz}(t)$, and
\begin{align}
\label{eq:sub}
X_{\enz:\subs}(t) = X_{\enz:\subs}(0)&+\pois_1(\int_{0}^t k_1 X_{\subs}(s)X_{\enz}(s)\der s)\\
& -\pois_2( \int_{0}^t k_2 X_{\subs:\enz}(s)\der s)\\
&-\pois_3( \int_{0}^t k_3 X_{\subs:\enz}(s)\der s),
\end{align}
and
\begin{align*}
X^{\volume}_{\subs}(t) = X^{\volume}_{\subs}(0) &-\frac{1}{\volume}\pois_1( \int_{0}^t k_1 \volume X^{\volume}_{\subs}(s)X_{\enz}(s)\der s)\\
&+\frac{1}{\volume}\pois_2(\int_{0}^t k_2 X_{\subs:\enz}(s)\der s)\\
= X^{\volume}_{\subs}(0) &-\frac{1}{\volume}\pois_1( \int_{0}^t \gamma_1 \volume X^{\volume}_{\subs}(s)X_{\enz}(s)\der s)\\
&+\frac{1}{\volume}\pois_2(\int_{0}^t \volume \gamma_2 X_{\subs:\enz}(s)\der s).
\end{align*}

We want to show that $\lim_{\volume\ra \infty} \hat{X}^{\volume}_{\product}(t) = \lim_{\volume\ra \infty}X^{\volume}_{\product}(t)$,
where $X^{\volume}(t) := \frac{X(t)}{\volume}$ and $\hat{X}^{\volume}(t) := \frac{X_{\product}(t)}{\volume}$.

Let $Z_{\subs}(t) = \frac{X_{\subs}(t)}{\volume}$. By diving the change for $X_E(t)$ with $\volume$ and taking the limit when $N\rightarrow \infty$, we obtain that
\begin{align*}
\lim_{\volume\ra \infty}\frac{X_{\enz:\subs}(t)}{\volume} = \lim_{\volume\ra \infty}[\frac{X_{\enz:\subs}(0)}{\volume}&+\frac{1}{\volume}\pois_1(\int_{0}^t \gamma_1 \volume X^{\volume}_{\subs}(s)X_{\enz}(s)\der s)\\
& -\frac{1}{\volume}\pois_2( \int_{0}^t {\gamma_2}{\volume} X_{\subs:\enz}(s)\der s)\\
& -\frac{1}{\volume}\pois_3( \int_{0}^t {\gamma_3}{\volume} X_{\subs:\enz}(s)\der s)],
\end{align*}
which, after applying the law of large numbers, amounts to
\begin{align*}
\int_{0}^t \gamma_1  X^{\volume}_{\subs}(s)X_{\enz}(s)\der s =  \int_{0}^t {(\gamma_2+\gamma_3)}{} X_{\subs:\enz}(s)\der s,
\end{align*}
implying that

\begin{align*}
X_{\subs:\enz}(s) = \hat{K} X^{\volume}_{\subs}(s) X_{\enz}(s) = \hat{K} X^{\volume}_{\subs}(s) (\enz_{T} - X_{\subs:\enz}(s)),
\end{align*}

and further

\begin{align*}
X_{\subs:\enz}(s) = \frac{\enz_{T}\hat{K} X^{\volume}_{\subs}(s)}{1+\hat{K} X^{\volume}_{\subs}(s)},
\end{align*}

from which it follows that $X_{\enz}(s) = \enz_T-X_{\subs:\enz}(s)$ equals
\begin{align*}
X_{\enz}(s) = \frac{\enz_{T}}{1+\hat{K} X^{\volume}_{\subs}(s)}.
\end{align*}

Finally, by substituting the obtained expression for $X_{\enz}(s)$ in \eqref{eq:sub}, we obtain that
\[
\deriv{X^{\volume}_{\subs}} = - \frac{\enz_{T}\gamma_3 \hat{K}}{1+\hat{K} X^{\volume}_{\subs}}.
\]

Finally, 




A complete proof is provided in \cite{kang2013separation}. 
We here sketch the general idea.

Our goal is to prove that the 

Let $Z_{\subs}(t) = X_{\subs}(t)/\volume$, $Z_{\enz}(t) = X_{\enz}(t)$, $Z_{\subs:\enz}(t) = X_{\subs:\enz}(t)$, $Z_{\product}(t) = X_{\product}(t)/\volume$.
Writing out the scaled random time-change model for the substrate gives:
\begin{align*}
Z_{\subs}(t) & = Z_{\subs}(0) - \volume^{-1}\pois_1(\volume \int_{0}^t \gamma_1 Z_{\subs}(s)Z_{\enz}(s)\der s)\\
&+\volume^{-1}\pois_2(\volume \int_{0}^t \gamma_1 Z_{\subs:\enz}(s)\der s),
\end{align*}
and writing out the scaled random time-change model for the enzyme gives:
\begin{align*}
Z_{\enz}(t) = Z_{\enz}(0) & - \pois_1(\volume \int_{0}^t \gamma_1 Z_{\subs}(s)Z_{\enz}(s)\der s)\\
& +\pois_2(\volume \int_{0}^t \gamma_2 Z_{\subs:\enz}(s)\der s)\\
&+\pois_3(\volume \int_{0}^t \gamma_2 Z_{\subs:\enz}(s)\der s)\\
%Z_{\subs}(t) & = Z_{\subs}(0) + \\
%Z_{\product}(t) & = Z_{\product}(0) +  \volume^{-1}\\
\end{align*}
Dividing the latter with $\volume$, after applying the law of large numbers gives the balance equations and implies the expression for $\frac{\der}{\der t} v_{\enz}(s)$.
The equation for $\deriv\conc{\subs}$ follows from the model of $Z_{\subs}(t)$, after applying the law of large number numbers and substituting  the obtained value of $\frac{\der}{\der t} v_{\enz}(s)$. 



%Whenever the rate of complex formation is much faster than the complex dissociation (i.e. $k_1\gg k_2+k_3$), the complex is formed 
%%\paragraph{Generalized enzymatic approximation - operator site reduction}
%This approximation is valid whenever the reaction of binding and unbinding between the substrate and the enzyme happens at a significantly faster time-scale than the conversion of the complex to the product. 
%%The situation arises either when the rate of conversion to the substrate is much larger than the rate of the conversion to the product ($k_1^-\gg\hat{k_1}$), or when the enzyme co

\subsubsection*{Generalized enzymatic reduction.}
The enzymatic approximation can be generalized to a situation where many sets of substrates compete for binding to the same enzyme.
%In this case, the rapid equilibrium approximation can be generalized in the following way.
Consider a sub-network of $n$ reactions where the $i$-th such reaction reads:
\begin{align*}
\enz+\subs_{i,1}+\ldots+\subs_{i,m_i} & \rates{k_i}{k_i^-} \enz:\subs_{i,1}:\ldots:\subs_{i,m_i} \rA{\hat{k_i}} \enz+\product_i. %\\
%\ldots\\
%\enz+\subs_{n2}+\ldots+\subs_{nm_n}& \rates{k_n}{k_n^-} \enz:\subs_{n1}:\ldots:\subs_{nm_n} \rA{\hat{k_n}} \enz+\product_n.
\end{align*}
The resulting approximation is
\begin{align*}
\subs_{i,1}+\ldots+\subs_{i,m_i}\rA{\frac{\hat{k_i}\enz_T K_1\conc{\subs_i}}{Z}} \product_i,
\end{align*}
where $\conc{\subs_i} = \prod_{j\in\{1,\ldots,m_i\}}\conc{\subs_{i,j}}$,  
$Z= 1+\sum_{j\in\{1,\ldots,n\}}\conc{\subs_j}$
and 
$\enz_T=\conc{E}(t)+\sum_{i=1}^n\conc{E:S_{i,1}:\ldots:S_{i,m_i}}(t)$. 
The latter expression follows from $\deriv \conc{E:S_{i,1}:\ldots:S_{i,m_i}}(t) =0$ for all $i=0,\ldots,n$.
%The validity of approximation is considered good when
%, or by 
%statistical thermodynamics.
%if $n$ reactions are competing for the same enzyme, and the system is at equilibrium, the probability that a particular enzyme will be in the $i$th configuration (out of the $n+1$ configurations in total) equals $\frac{\hat{k_i} K_1[X_i]}{Z}$ for $i=1,\ldots,n$ and equals $\frac{1}{Z}$ for a configuration of free enzyme.


\subsubsection*{Fast dimerisation reduction.}
Finally, consider the dimerisation reaction $M+M\rates{k}{k^-} M_2$ and assume that $\deriv \conc{M}(t) = k\conc{M}(t)^2-k^-\conc{M_2}(t)=0$.
As a consequence, the dimerisation reaction itself can be eliminated, and the monomer and dimer concentrations which can be expressed as a fraction of the total concentration of molecules $M$:
\begin{align*}
\conc{M}(t)  = \frac{1}{4K} \left(\sqrt{8K\conc{M_T}+1} -1 \right),\;\;\;\hbox{     and     } \;\;\; \\
\conc{M_2}(t)  = \frac{M_T}{2}-\frac{1}{2}\conc{M}(t),
\end{align*}
where $M_T = \conc{M}(t)+2\conc{M_2}(t)$.
%In our model, operator site will take the role of the enzyme.



==> tex/fig-eventcount.tex <==
\begin{figure}[t]
\begin{center}
\includegraphics[scale=0.5]{Figures/eventcount.png}
%\includegraphics[scale=0.35]{Figures/eventratio.pdf}
\end{center}
\caption{
%
The average number of events per simulation (after each of the reduction steps separately, and for a fully reduced model). 
%
The operator-site reduction has the largest reduction in the transient (until around $500$ steps), 
but the dimerisation reduction provides the best result in the whole cell cycle.
%
The combination of the two reductions results in a significantly reduced number of events.
}
\label{fig:eventcount}
\end{figure}


==> tex/fig-eventratioconzelmann.tex <==
\begin{figure}[t]
\begin{center}
\includegraphics[scale=0.5]{Figures/eventratioconzelmann.pdf}
\end{center}
\caption{..}
\label{fig:eventratioconzelmann}
\end{figure}


==> tex/packages.tex <==
\usepackage{graphicx} % support the \includegraphics command and options
\usepackage{stmaryrd}
\usepackage{url}
%\usepackage{va}
\usepackage{frcursive}
\usepackage{calligra} 
%\usepackage{la}
%\usepackage[T1]{fontenc}
%\usepackage{mathpazo}
%\usepackage{unicode-math}
%\usepackage{calrsfs}
%\usepackage[ruled, vlined]{algorithm2e}
\usepackage{latexsym}
%\usepackage{caption}
\usepackage{graphicx}
%\usepackage{calrsfs}
\usepackage{mathrsfs}
% \usepackage[parfill]{parskip} % Activate to begin paragraphs with an empty line rather than an indent

%%% PACKAGES
%\usepackage{geometry} % to change the page dimensions
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{amsbsy}
\usepackage{amsthm}
\usepackage{setspace}
\usepackage{MnSymbol} 
\usepackage[ruled, vlined]{algorithm2e}
%\usepackage{graphicx}
%\usepackage{MnSymbol} 
%\usepackage{multicol}
\usepackage{color}
%\usepackage{subfigure} 
%\usepackage[lined,commentsnumbered]{algorithm2e} %
%\usepackage{booktabs} % for much better looking tables
%\usepackage{array} % for better arrays (eg matrices) in maths
%\usepackage{paralist} % very flexible & customisable lists (eg. enumerate/itemize, etc.)
\usepackage{verbatim} % adds environment for commenting out blocks of text & for better verbatim
%\usepackage{subfig} % make it possible to include more than one captioned figure/table in a single float
% These packages are all incorporated in the memoir class to one degree or another...

\usepackage{amsmath}
\usepackage{amssymb} 
\usepackage{amsfonts,epsfig,graphicx,enumitem,multicol} 
%\usepackage{graphicx}
%\usepackage{MnSymbol} 
%\usepackage{multicol}
\usepackage{color}

==> tex/table-results.tex <==


\begin{table}
\begin{center}
\begin{tabular}{l|l|l|l}
\hline\noalign{\smallskip}
 Reduction & Rules & Proteins
  &  Simulation time\\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
 Initial model & 96 & 16 %(+61 species) 
 & $\approx$40 mins \\
 \hline
 E(nzymatic) & 92 & 14 %(+57 species) 
 & $\approx$ 40 mins \\
 \hline
 E + O(perator)& 36 & 6 %(+0 species) 
 & $\approx$ 20 mins \\
\hline
E + O + D(imerization)&34&6 %(+0 species)
& $\approx$ 20 secs\\
\hline
E + O + D + M(odifier elim.)&34&5 %(+0 species)
&$\approx$ 15 secs\\
\hline
E + O + D + M + S(imilar reac. comb.) &11&5 %(+0 species)
&$\approx$5 secs\\
\hline
\label{table:compare}
\end{tabular}
\caption{Comparison of model size and simulation speed at intermediary steps of the reduction algorithm.}
\end{center}
\end{table}


